Exploring Opportunistic Meta-knowledge to Reduce Search Spaces for Automated Machine Learning

Machine learning (ML) pipeline composition and optimisation have been studied to seek multi-stage ML models, i.e. preprocessor-inclusive, that are both valid and well-performing. These processes typically require the design and traversal of complex configuration spaces consisting of not just individual ML components and their hyperparameters, but also higher-level pipeline structures that link these components together. Optimisation efficiency and resulting ML-model accuracy both suffer if this pipeline search space is unwieldy and excessively large; it becomes an appealing notion to avoid costly evaluations of poorly performing ML components ahead of time. Accordingly, this paper investigates whether, based on previous experience, a pool of available classifiers/regressors can be preemptively culled ahead of initiating a pipeline composition/optimisation process for a new ML problem, i.e. dataset. The previous experience comes in the form of classifier/regressor accuracy rankings derived, with loose assumptions, from a substantial but non-exhaustive number of pipeline evaluations; this meta-knowledge is considered 'opportunistic'. Numerous experiments with the AutoWeka4MCPS package, including ones leveraging similarities between datasets via the relative landmarking method, show that, despite its seeming unreliability, opportunistic meta-knowledge can improve ML outcomes. However, results also indicate that the culling of classifiers/regressors should not be too severe either. In effect, it is better to search through a 'top tier' of recommended predictors than to pin hopes onto one previously supreme performer.

==> backup (210112)/0.abstract.tex <==
\begin{abstract}


Machine learning (ML) pipeline composition and optimisation have been studied to find valid and well-performing pipelines.
ML pipeline composition and optimisation requires to design configuration spaces including ML components, their hyperparameters and pipeline structures to link these components. 
Reducing configuration spaces by ignoring low-performing ML components enables ML pipeline composition and optimisation methods to explore these configuration spaces faster to find better ML pipelines.
This paper investigates the impact of configuration space reduction using the relative landmarking method taking into account and considering a certain level of reliability of the meta-knowledge base generated from prior evaluations. To design a configuration space for a new problem, the top \textit{k} well-performing ML components of the most similar previously solved problem are used to design the configuration space for the new problem.
%The experiments show the effectiveness of the relative landmarking method in reducing configuration spaces by selecting a reasonable value of \textit{k}.
The experiments show that the most reasonable value of \textit{k} is 10 that is equivalent to the reduction of the full configuration space by 67\%. Moreover, the extreme value of \textit{k}=1 does not construct well-performing configuration spaces due to the uncertainty of the meta-knowledge base.









\end{abstract}

==> backup (210112)/1.introduction.tex <==

\section{Introduction}
\label{sec:intro}


Various ML pipeline composition and optimisation methods have been proposed in recent years to find valid and well-performing pipelines given both a problem (i.e., a dataset) and a set of ML components with tunable hyperparameters \cite{sabu18,zohu19,ngma20,kemu20}. 
One of the most successful ML pipeline composition and optimisation methods is based on a sequential model-based optimisation (SMAC) approach \cite{thhu13}. The key idea of this method is to find a balance between the exploration and exploitation of configuration spaces. The exploitation searches for ML pipelines that are similar to the current best-performing pipelines in terms of pipeline structures and values of hyperparameters, whereas the exploration randomly searches for pipelines within the configuration spaces to escape the local optimum potentially emerging from the exploitation part of the optimisation process. 
There are several automated machine learning (AutoML) tools that implement SMAC. AutoWeka version 0.5 \cite{thhu13} implements SMAC to search for one-component pipelines. The configuration spaces of AutoWeka 0.5 include only predictors and their hyperparameters. AutoWeka4MCPS extends the configuration spaces with the data preprocessing components to construct multiple-component pipelines \cite{sabu18}.
This extension of the configuration space has a potential for exploration of a wider range of diverse, well performing ML pipelines but does come with a number of challenges.
One of key challenges of large configuration spaces is that it is more difficult and requires more time to find valid and well-performing pipelines. 
There is therefore a need and great interest in approaches offering intelligent reduction of the configuration spaces by only selecting promising well-performing ML components. Such a reduction has a crucial advantage of allowing the ML pipeline composition and optimisation methods to work in and explore smaller configuration spaces which are constructed from the most suitable and well-performing ML components.


There have been several attempts to deal with the problem of configuration space reduction using two main approaches, predefined pipeline structures and meta-learning. Firstly, the approach using predefined pipeline structures reduces configuration spaces by defining fixed structures \cite{sabu18,fekl15}, or ad-hoc specifications \cite{depi17,tsga12,olmo16,wemo18,giya18} (e.g., context-free grammars) to construct pipelines based on experts' knowledge. A drawback of this approach is the potential bias of experts' knowledge used to construct such fixed pipeline structures. Therefore, it potentially limits the opportunity to find better pipelines residing outside of such predefined templates or structures. 
Secondly, the approach using meta-learning reduces the configuration spaces by learning from prior evaluations. Configuration spaces are reduced by selecting top well-performing components \cite{dbbr18,va19,lebu15,albu15}, important hyperparameters and ranges of these hyperparameters for a given problem \cite{albu15,rihu18,prbo19,wemu20}.
This approach requires intensive evaluations of many ML components, their hyperparameters and many datasets that have diverse characteristics \cite{lega10,lega10a,albu15}. Because of the computational challenges, previous studies only investigated the importance of hyperparameters for up to six algorithms \cite{rihu18,prbo19,wemu20}.
Therefore, generating a very reliable meta-knowledge base from prior evaluations is very difficult. 
On account of the fact that we usually have prior evaluations resulting from executing automated ML pipeline composition and optimisation methods, we would like to address the research questions about how many and which ML components we should select to design configuration spaces acknowledging and taking into account a certain level of accuracy and reliability of a meta-knowledge base generated from such prior evaluations.
Our study employs the relative landmarking method \cite{va19} to reduce configuration spaces. We construct a meta-knowledge base from prior evaluations of two-hour ML pipeline composition and optimisation of SMAC over 20 datasets. The meta-knowledge base contains the mean error rate of ML components for each prior dataset.   
The new dataset is evaluated by executing a certain number of landmarkers (i.e., single-component pipelines). The performance of the landmarkers on the new dataset is correlated with the performance of these landmarkers on prior datasets from the meta-knowledge base. The top \textit{k} well-performing ML components of the most similar dataset are selected to construct configuration spaces. 
To this end, this study has two main contributions:

\begin{itemize}
    \item A definition of the problem of ML pipeline composition and optimisation with dynamic configuration spaces.
    
    \item A study of the impact of the levels of the configuration space reduction (i.e., specified by different values of \textit{k}) on the performance of ML pipeline composition and optimisation methods given a certain level of reliability of the meta-knowledge base.
    
    
\end{itemize}




This paper is divided into 6 sections. After the Introduction,
Section \ref{sec:related_work} presents previous studies to reduce configuration spaces in the context of AutoML.
Section \ref{sec:search_space_modelling} presents the definition of the problem of ML pipeline composition and optimisation with dynamic configuration spaces.
Section \ref{sec:relative_landmarking} presents the methodology of using the relative landmarking method to reduce configuration spaces.
Section \ref{sec:experiment} presents experiments to investigate the problem of configuration space reduction. Finally, Section \ref{sec:conclusion} concludes this study.
 


==> backup (210112)/2.related_work.tex <==
\section{Related Work}
\label{sec:related_work}


The growing number of available ML methods with their often complex hyperparameters leads to a very quick expansion of the ML pipelines configuration options and spaces. Intelligent reduction of these configuration spaces enables the ML pipeline composition and optimisation methods to find valid and well-performing ML pipelines faster given typical constraints of execution environments and time budget.
We review two main approaches to reduce the configuration spaces in the context of ML pipeline composition and optimisation. 

\textit{Predefined ML pipeline structures and components' hyperparameters:} This approach can be implemented as fixed pipeline templates \cite{sabu18,fekl15} or ad-hoc specifications \cite{depi17,tsga12,olmo16,wemo18,giya18} such as context-free grammars. Moreover, specific ranges of hyperparameters' values, which highly contribute to well-performing pipelines, are also predefined in these specifications.
The advantage of this approach is to reduce configuration spaces by restricting the length of ML pipelines, ML components and orders of these components based on experts' knowledge. However, the disadvantage of this approach is that there might be very well performing ML pipelines outside of the predefined templates. 


\textit{Meta-learning:} This approach aims to reduce configuration spaces by learning the characteristics of prior evaluations. The main idea of this approach is to establish relationships between datasets' characteristics and the performance of ML components based on prior evaluations \cite{dbbr18,lebu15,lega10,albu15}. The representations of datasets' characteristics can be meta-features or the relative performance of landmarkers. The landmarkers are usually one-component pipelines that are used to evaluate the performance of ML components.  The meta-learning approach can be used to reduce configuration spaces by selecting a number of well-performing ML components  \cite{albu15,dbbr18,va19,lebu15} or important hyperparameters for tuning \cite{albu15,rihu18,prbo19,wemu20}. To select top well-performing pipelines, \textit{average ranking} and \textit{active testing} were used to recommend one-component pipelines for new datasets \cite{dbbr18}. However, these approaches have not been applied to AutoML yet. Moreover, these studies limit their scopes by searching for one-component pipelines.
To perform the hyperparameter optimisation for the recommended one-component pipelines, these studies also use the grid search that has been proven to be not as effective as SMAC \cite{thhu13}. 
The previous studies have also investigated the importance of hyperparameters \cite{rihu18,prbo19,wemu20} from prior evaluations. 
An important hyperparameter can contribute to a high variance of the performance (i.e., error rate) of an ML algorithm. For example, gamma and complexity are the most important hyperparameters of SVM \cite{rihu18}.
The results of these studies can be used to reduce configuration spaces by removing less important hyperparameters (i.e., set default values to less important hyperparameters) and less important ranges of hyperparameter values.  
This reduction of configuration spaces enables ML pipeline composition and optimisation methods to dedicate more time to searching for the best values of the important hyperparameters as they have the highest impact on finding well-performing pipelines.
A disadvantage of these studies is that the importance of hyperparameters of ML components is studied on small sets of algorithms (i.e., up to 6 algorithms). The reason is that it is extremely challenging and time-consuming to evaluate all possible hyperparameters of available algorithms. 

Being different from these approaches, our approach acknowledges and accepts a certain level of reliability of prior evaluations which are used to build a meta-knowledge base. We use the relative landmarking method to select well-performing ML components to construct configuration spaces for the ML pipeline composition and optimisation. We also investigate the impact of the levels of the configuration space reduction on the performance of ML pipeline composition and optimisation methods.


==> backup (210112)/3.search_space_modeling.tex <==

\section{Modelling Configuration Spaces for ML Pipeline Composition and Optimisation }
\label{sec:search_space_modelling}

To control the extension and reduction of configuration spaces in the context of AutoML, we model configuration spaces using a generic tree structure. After that, we extend the problem of pipeline composition and optimisation \cite{sabu18} by adding a factor representing pipeline structures. Finally, we define the problem of pipeline composition and optimisation with dynamic configuration spaces as a constraint optimisation problem.



\subsection{Configuration Space Modelling}


Given a tree-structured set of nodes $\mathcal{X}$ and a set of ML components $\mathcal{A}$, for each tree node $x_i \in \mathcal{X}$:


\begin{equation}
\small{
x_i=(\mathcal{A}_i,\lambda_i, \epsilon_i)
\label{eq:treenode}
}
\end{equation}

where $\mathcal{A}_i$ is an ML component, $\lambda_i$ is the set of hyperparameters for component $\mathcal{A}_i$, and $\epsilon_i$ represents the active/inactive status of this node. If a node is a predictor and has the inactive status, all of its children node are recursively inactive.



A tree-based configuration space $\mathcal{T}$ is defined as: 

\begin{equation}
\small{
\mathcal{T}=(\mathcal{X},f_p)
\label{eq:searchtree}
}
\end{equation}

Function $f_p$ assigns each node $x_i$ to a parent node $f_p(x_i)$. A root node has $x_i=f_p(x_i)$. 

Each ML pipeline $p$ is a search path constructed by back tracking from an active leaf node to the root node.  

\begin{equation}
\small{
p = (g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})
\label{eq:pipeline}
}
\end{equation}

where $g$ is a sequential pipeline structure which defines how the components are connected, $\vec{\mathcal{A}}\in \mathcal{A}$ is a vector of the selected components, $\vec{\mathcal{\lambda}}\in \mathcal{\lambda}$ is a vector of hyperparameters of all selected components. A pipeline $p$ can also be called a configuration.
Configuration spaces can be extended by adding tree nodes, or reduced by deactivating tree nodes which form invalid and bad-performing pipelines.




\subsection{The Problem of Pipeline Composition and Optimisation With Dynamic Configuration Spaces}


The problem of pipeline composition and optimisation is to find the most promising machine learning pipeline $(g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{*}$ including pipeline structures, selected components and their hyperparameters. The definition of this problem is extended from \cite{sabu18} as:

\begin{equation}
\small{
(g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{*} = argmin\frac{1}{k}\sum_{i=1}^{k} \mathcal{L}((g,\vec{\mathcal{A}},\vec{\mathcal{\lambda}})^{(i)},\mathcal{D}^{(i)}_{train},\mathcal{D}^{(i)}_{valid})
}
\label{eq:pipeline_problem}
\end{equation}

where $\mathcal{D}_{train}$ and $\mathcal{D}_{valid}$ are training and validation datasets. Equation \ref{eq:pipeline_problem} minimises k-fold cross validation error of the loss function $\mathcal{L}$.




Equation \ref{eq:pipeline_problem} does not consider changes of the configuration space $\mathcal{T}$. If we reduce this configuration space by selecting promising well-performing pipelines to form the configuration space $\mathcal{T}^{*}$, the problem of pipeline composition and optimisation can be extended as a constraint optimisation problem as follows:  


\begin{equation}
\small{
(g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{*} = argmin\frac{1}{k}\sum_{i=1}^{k} \mathcal{L}((g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{(i)} \in \mathcal{T}^{*},\mathcal{D}^{(i)}_{train},\mathcal{D}^{(i)}_{valid})
}
\label{eq:extended_pipeline_problem}
\end{equation}

\textit{subject to}


\begin{equation}
\small{
\mathcal{T}^{*} \subset \mathcal{T} \:\:\:\:\:  \textit{and} \:\:\:\:\:  h(\mathcal{T}^{*}) = \emptyset 
\label{eq:extended_pipeline_problem_constraints_1}
}
\end{equation}


where $h(\mathcal{T}^{*})$ is a function to find invalid pipelines. 




==> backup (210112)/4.relative_landmarking.tex <==

\section{Configuration Space Reduction Using the Relative Landmarking Method}
\label{sec:relative_landmarking}

In this section, we present the methodology to design configuration spaces for the ML pipeline composition and optimisation given the meta-knowledge base of uneven quality and certain level of uncertainty. A relative landmarking method, inspired by the \textit{average ranking} \cite{dbbr18} and the \textit{relative landmarking} \cite{va19} approaches, is proposed. These methods are used to recommend an ML algorithm for a given dataset though they have not considered the optimisation time budget or have been proposed in the context of the automated composition and optimisation of ML pipelines which are both the subject of our primary investigations. 
Besides, there exists an uncertainty in the meta-knowledge base, which describes the relationships between the average performance of ML components and the datasets' characteristics. 
This uncertainty is due to the lack of a thorough evaluation which covers the combined effects of ML components in pipelines, the diversity of pipeline structures and components' hyperparameters.
To be more specific, because the meta-knowledge base is generated from prior evaluations of the automated composition and optimisation, the number of times, that ML components are evaluated, is different. There are even those that have not been evaluated or have been evaluated with a small number of times due to the limit of the optimisation time budget.
Such thorough evaluations to generate highly reliable meta-knowledge are prohibitively expensive in the context of ML pipeline composition and optimisation task and we are interested in investigating if at all and how partial or less reliable meta-knowledge can be effectively used in our context.
    

Firstly, we present the problem formulation of configuration space reduction using the relative landmarking method. Secondly, we present landmarkers that are used to evaluate a new dataset to understand its characteristics. Thirdly, we present the algorithm to design configuration spaces given a new dataset and prior evaluations on other problems from which, we assume, a useful knowledge can be extracted.




\subsection{Problem Formulation}
\label{sec:problem_formulation}


We define the problem of pipeline composition and optimisation with dynamic configuration spaces in Equation \ref{eq:extended_pipeline_problem}. An optimal configuration space $\mathcal{T}^{*}$ can be designed at the initialisation of the ML pipeline composition and optimisation methods. The configuration space $\mathcal{T}^{*}$ of the new dataset is constructed by \textit{k} best performing ML components of the most similar dataset from prior evaluations.

Given a new dataset $t_{new}$, we need to find a prior dataset $t^{*}_{i}$ which is similar to $t_{new}$ \cite{va19}. In order to do that, we evaluate a set of landmarkers (i.e., pipelines) $\Theta=\{\theta_i\}$  on $t_{new}$ and record their performance results $E_{new}$. We measure the relative similarity of the performance of the landmarkers between the new dataset $t_{new}$ and the prior dataset $t_{i}$. We select the most similar dataset $t^{*}_{i}$ based on the ranking of the similarity. The configuration space  $\mathcal{T}_{new}$ of the dataset $t_{new}$ is constructed by selecting the top $k$ well-performing ML components of the previously tackled dataset $t^{*}_{i}$.



\subsection{Landmarkers}

Landmarkers \cite{va19} $\Theta=\{\theta_i\}$ are the ML methods/pipelines. They are usually simple and efficient to execute. 
They are used to indirectly evaluate the characteristics of datasets through  evaluations of their performance (e.g., classification accuracy) which can then be used as meta-features.
These meta-features are used to find the most similar previously solved dataset by matching the relative performance of the landmarkers on the new dataset and the previously solved datasets.
Selecting a set of landmarkers, or more generally a set of meta-features describing complex problems, obviously has an impact on the final results as shown in a number of previous studies on the subject \cite{va19,albu15}. As in the context of AutoML, the evaluation time of the landmarkers forms a part of the overall AutoML optimisation time, in this study we have made a deliberate decision to evaluate a limited set of landmarkers which are the fastest to execute. Therefore in our experiments we use the five fastest predictors (i.e., RandomTree, ZeroR, IBk, NaiveBayes and OneR) from the compiled ranking of the average evaluation time of the pipelines containing these components in prior evaluations. We acknowledge that this choice is not optimal in any other sense than their cumulative execution time but it is a part of our study goals whether such a crude approach for complex problems matching could still be effective, and to what extent, in reduction of our input search space for AutoML algorithms.



\subsection{Dynamic Configuration Space Design}



\begin{algorithm}[!htbp]
\small

\caption{\small Design Configuration Space Using The Relative Landmarking}
\begin{algorithmic}[1]
\Require
      \Statex $\Theta$: The set of landmarkers
      \Statex $t_{new}$: The new dataset
      \Statex $t_{prior}$: The prior dataset
\Statex      
\For{$\theta_i$ \textbf{in}  $\Theta$}
        \State $E_{new}\_i$ = \textit{evaluate}($\theta_i$, $t_{new}$)
\EndFor
\For{\textbf{each}  $t_{prior}\_i$}
        \State $correlation\_coefficient_i$ = 
        
        \textit{calculateCorrelation}($E_{new}$, $E_{prior}\_i$)
\EndFor
\State $t^{*}$ = \textit{getMostSimilarTask}($correlation\_coefficient$) 
\State $\mathcal{T}_{new}$ = \textit{selectMLComponents}($t^{*}$, $k$)
\State \textbf{return} $\mathcal{T}_{new}$
\end{algorithmic}
\label{algorithm:construct_configuration_space}
\end{algorithm} 




Algorithm \ref{algorithm:construct_configuration_space} presents the algorithm to design a configuration space using the relative landmarking method. This configuration space is used as an input for AutoML pipeline composition and optimisation methods. Firstly, the algorithm evaluates the new dataset $t_{new}$ using each landmarker $\theta_i$. The result is the performance $E_{new}\_i$ (e.g., the 10-fold cross-validation error rate) of this landmarker (line 1-3). Secondly, the algorithm calculates Pearson correlation coefficient of $E_{new}\_i$ with the mean error rate of the landmarkers on previously solved datasets $E_{prior}\_i$ (line 4-6). Thirdly, the algorithm ranks the correlation coefficients and selects the dataset $t^{*}$ that has the highest correlation coefficient (line 7). Finally, the configuration space is constructed by all preprocessing components and top \textit{k} best performing predictors (line 8) of the most similar dataset $t^{*}$. Note that sum of the evaluation time of landmarkers on the new dataset is deducted from the total time budget of the ML pipeline composition and optimisation task.

==> backup (210112)/5.experiments.tex <==
\section{Experiments}
\label{sec:experiment}

In the experiments, we use the method described in Section \ref{sec:relative_landmarking} to explore the impact of the levels of configuration space reduction on the performance of AutoML composition and optimisation method. 
To do so, we compare the mean error rate of five approaches to design the configuration spaces:

\begin{itemize}
    \item \textbf{baseline}: The full configuration space as is constructed by the preprocessing and predictor components that are implemented in AutoWeka4MCPS \cite{sabu18}. The reduction of configuration spaces is effective only if this reduction enables SMAC to find better pipelines than using the baseline configuration space.
    
    \item \textbf{r30}: A restricted configuration space using fixed pipeline structures extracted from the best pipelines found within 30 hours optimisation time \cite{sabu18}. By using this configuration space, the AutoML composition and optimisation method dedicates time to optimise hyperparameters of the fixed ML pipelines. We use this configuration to illustrate the trade-off between only optimising hyperparameters of fixed complex pipelines and searching for both well-performing pipeline structures and their hyperparameters within the reduced configuration spaces.
    
    
    \item \textbf{avatar}: The full configuration space which is similar to the \textbf{baseline} configuration space, but we use the AVATAR\cite{ngma20} to reduce configuration spaces by quickly ignoring invalid pipelines when using SMAC to exploit and explore the baseline configuration space. 
    
    
    \item \textbf{oracle settings (\textit{O-k1}, \textit{O-k4}, \textit{O-k8}, \textit{O-k10}, and \textit{O-k19})}: The oracle configuration spaces designed by selecting k (i.e., k in $\{1,4,8,10,19\}$) predictors which have the lowest mean error rate in prior evaluations for the datasets themselves.
    The purpose of using oracle settings is to demonstrate that even if we ignore the impact of using the landmarking method to find the most similar prior problem, the meta-knowledge base which is generated from prior evaluations of AutoML composition and optimisation is useful and meet a certain level of reliability to be used for the reduction of configuration spaces.
    
    
    
    
    \item \textbf{landmarking settings (\textit{L-k1}, \textit{L-k4}, \textit{L-k8}, \textit{L-k10}, and \textit{L-k19})}: The relative landmarking configuration spaces designed by selecting k (i.e., k in $\{1,4,8,10,19\}$) predictors which have the lowest mean error rate in prior evaluations of the most similar dataset using the relative landmarking. We use the landmarking settings for the experiment to show that how much should we reduce configuration spaces if there exists uncertainties of both the meta-knowledge base and the matching method (i.e., the landmarking method) we use the find the most similar prior problems.
    
    
    
    
\end{itemize}


\subsection{Experimental settings}

For the experiments we will use a variety of datasets which are presented in Table \ref{tab:datasets}.
The AutoML tool we use for the experiments is AutoWeka4MCPS\footnote{https://github.com/UTS-AAi/autoweka} which implements the method of configuration space reduction using the relative landmarking.
The ML pipeline composition and optimisation method is SMAC. 
We also use the AVATAR to evaluate the validity of ML pipelines \cite{ngga20} which dynamically reduces configuration spaces by ignoring invalid pipelines which are generated during the exploration and exploitation of SMAC.
We set the time budget to 2 hours and the memory to 1GB.
We perform five runs of experiment for each dataset and report the mean error rate of the best pipelines found.  
We use the leave-one-out strategy for the experiments with regard to the meta-data availability.
For each dataset, we exclude the prior evaluations of this dataset from the meta-knowledge base when performing the relative landmarking method to reduce configuration spaces. The optimisation time for SMAC in cases of using the relative landmarking method is the remaining time of 2 hours after using the landmarking method to construct the configuration spaces. 

We have conducted a preliminary study to investigate the feasibility of configuration space reduction using the relative landmarking method  by extracting prior evaluations. We use Algorithm \ref{algorithm:construct_configuration_space} to design configuration spaces for each dataset.
We extract the prior evaluations of the most similar dataset found using the relative landmarking method. The extracted evaluations exclude pipelines that are not in the reduced configuration spaces. We make an assumption that these extracted evaluations are the results of the ML pipeline composition and optimisation without running the optimisation tasks that are time-consuming.
By doing so, we have to accept an issue that the total optimisation time of the extracted evaluations is less than total budget time (i.e., 2h). However, we can quickly select a subset of \textit{k} which is used to perform both the configuration space reduction as well as the pipeline composition and optimisation with the reduced configuration spaces.
For each dataset, we compare the ranking of predictors of different reduced configuration spaces \textit{k-space} and the configuration space constructed by selecting the top 8 well-performing predictor components of all datasets (\textit{avg-k8}).
The size of \textit{avg-k8} is approximately 25\% of the full configuration space.
We select 8 components for this exploratory study because we expect the landmarking method is effective when it comes to constructing a configuration space consisting of ML components which are better than the top 25\% average well-performing components from all prior evaluations.


Figure \ref{fig:k_Values} shows the number of cases (i.e., datasets) with the ranking of the best ML component in \textit{k-space} is higher than or equal the one in \textit{avg-k8} (metric-k). We can see that \textit{metric-k} increases when the value of \textit{k} increases because of the increase of the possibility for the best ML component being among the \textit{k} selected components. We choose 5 values of \textit{k} (i.e., 1, 4, 8, 10 and 19) to generate the configuration spaces and run the ML pipeline composition and optimisation tasks using these configuration spaces. We choose these values of \textit{k} because of the following reasons:

\begin{itemize}
    \item The value of k=1 is with the minimum configuration space.
    \item The values of k from 19 to 30 have the same \textit{metric-k}. The values of k from 10 to 18 also have the same \textit{metric-k}. We choose the smallest value of k=19 and k=10 because we want to maximise the reduction of configuration spaces.
    \item The values of k=4 and k=8 were chosen as they are between k=1 and k=10 so offer the best coverage of the space.
\end{itemize}




%\vspace{-0.60cm}
\begin{figure*}[htbp]
\centering
\includegraphics[width=0.95\linewidth]{images/exp1_k_values.pdf}
\caption{The number of cases (i.e., datasets) with the ranking of the best ML component in \textit{k-space} is higher than or equal the one in \textit{avg-k8} (metric-k).}
\label{fig:k_Values}
\end{figure*}


\input{tables/tab_dataset}
%\include{tables/tab_histotical_runs_predictors_and_ranking_mean_error}



%\subsection{Investigate the impact of selecting different values of k of the relative landmarking}

\subsection{Experiment Results}


%move to supplementary documents
\input{tables/tab_error_all_methods}
\input{tables/tab_pipelines_apart}

%\include{tables/tab_pipelines_1}
%\include{tables/tab_error_all_methods_ranking}
%\input{tables/tab_pipelines_2}
%\include{tables/tab_pipelines_3}




%\input{tables/tab_landmarking_results_extractedhistory}



%To facilitate the study, we use prior evaluations of AutoWeka4MCPS with 2 hours optimisation time, 1GB memory, using SMAC as the ML pipeline composition and optimisation method over 20 datasets. 
%We extracts the mean error rate of predictors based on the error rate of their ML pipelines within 20 datasets in the prior evaluations. Based on the mean error rate of the predictors, we generate the ranking of predictors across 20 datasets, as shown in Figure \ref{fig:ranking_predictors}. We can see that there is no predictor has the best ranking across all datasets. For example, the component \textit{Logistic} has the top ranking in the cases of the datasets \textit{abalone}, \textit{semeion} and \textit{waveform}. However, this component ranks 19\textsuperscript{th} and 26\textsuperscript{th} in the case of the datasets \textit{convex} and \textit{secom}.



Table \ref{tab:error_rate_all_methods} presents the mean error rate (\%) of the best pipelines found by SMAC using different methods to design configuration spaces.
The lowest mean error rate for each dataset is shown in bold. The `-' symbol represents a ``not found'' solution due to incomplete runs within the optimisation time. Figure \ref{fig:cd_diagram} shows the critical difference diagram of the average rankings of the mean error rate with different configuration spaces.
Table \ref{tab:pipelines}\footnote{The details of the best ML pipelines found by SMAC with different configuration spaces for all data sets can be found at \url{https://github.com/UTS-AAi/autoweka/blob/master/autoweka4mcps/doc/landmarking_supplementary.pdf} } shows the best ML pipelines found by SMAC with different configuration spaces for the data sets \textit{amazon} and \textit{convex}. .


\begin{figure}[h] 
    \centering
    \includegraphics[width=0.8\linewidth]{images/cd_all_methods.pdf}
    \caption{The critical difference diagram of the average ranking of the performance of SMAC with different configuration spaces.}
    \label{fig:cd_diagram}
\end{figure}

\begin{figure}[h] 
\includegraphics[width=1.00\linewidth]{images/mlcomponent_ranking_part.pdf}
\caption{The ranking of ML predictor components based on mean error rate of their pipelines from prior evaluations for selected datasets.}
\label{fig:ranking_predictors}
\end{figure}


\textit{Extreme values of \textit{k}=1 and k=19:} We can see that the values of \textit{k} that resulted in the worst performance is 1 and 19 in both cases of the relative landmarking and the oracle. We can also see that when selecting \textit{k} equals 1 (i.e., \textit{L-k1} and \textit{O-k1}), SMAC finds pipelines that have the lowest error rate of 5 in 20 datasets that is higher than using other configuration spaces.
Moreover, the number of incomplete optimisation tasks of \textit{L-k1} and \textit{O-k1} is 5 and 4 respectively that is also higher than the other methods. The reason is that the selection of the extreme value of \textit{k}=1 can reduce the configuration spaces significantly. If the relative landmarking method can recommend a well-performing predictor component accurately, SMAC can spend more time for the hyperparameter optimisation of pipelines containing this ML component. 
Therefore, the extreme selections of k1 have more chance to find the well-performing pipelines. However, SMAC does not have an opportunity to explore other solutions in cases the selected predictor component, which is recommended by the relative landmarking, is not well-performing due to the lack of thorough evaluations of this component. For example, for the dataset \textit{amazon}, \textit{L-k1} has the highest error rate which has the configuration space constructed from \textit{Logistic}. However, the pipeline that has the minimum mean error rate is a pipeline containing \textit{NaiveBayesMultinominal}. We also see that for the datasets \textit{abalone, adult, car, dexter} and \textit{waveform}, \textit{L-k1} has the lowest mean error rate although the average ranking \textit{L-k1} is only better than the cases using the full configuration space (i.e., \textit{baseline}). 
The selection of k19 makes its configuration space to be larger than ones of k1, k4, k8 and k10. Therefore, SMAC has less time for the hyperparameter optimisation. It is even worsen than using the full configuration spaces if the top predictors are not selected into the configuration spaces due to the uncertainty of the meta-knowledge base. The average ranking of \textit{L-k19} is slightly better than \textit{L-k1} and \textit{baseline}, 8.25 compared with 8.80 and 9.65 (Figure \ref{fig:cd_diagram}).


\textit{The middle values of k=4, k=8 and k=10}: The selection of k4, k8 and k10 can construct a better configuration spaces than the extreme values k1 and k19. It can avoid the extreme selection of only one predictor component which may not be well-performing, as well as the design of large configuration spaces which are difficult to be explored within a time budget.
Figure \ref{fig:cd_diagram} shows that \textit{L-k10} is critically different from the \textit{baseline} configuration space, 5.50 compared with 9.56. In other words, the relative landmarking with k10 can effectively reduce the configuration spaces to enable the ML composition and optimisation method to find better pipelines. 



\textit{The case of the dataset \textit{convex}:} In the case of using the fixed pipeline from the 30-hour optimisation (r30), the best pipeline structure is \textit{RandomForest} $\rightarrow$ \textit{AdaBoostM1} having the mean error rate 18.47 that is reported from the study of Savaldor et al. \cite{sabu18}. However, our experiment shows that the mean error rate of using \textit{r30} with 2-hour optimisation in case of \textit{convex} is 46.72.  
The best pipeline structure of the other settings has only one component. L-k10 and O-k8 have the lowest mean error rate (i.e., 25.65 and 25.51). The best pipelines of L-k10 and O-k8 are \textit{RandomForest} and \textit{SMO} respectively. It clearly shows that performing hyperparameter optimisation for a complex pipeline may not produce a well-performing pipeline in comparison with performing AutoML composition and optimisation using reduce configuration spaces (i.e., in the cases of O-k1, O-k4, O-k8, O-k10, O-k19, L-k8 and L-k10). 
The reason is that it takes more time to optimise hyperparameters of a complex pipeline and the given time budget is not enough. In these cases, performing AutoML composition and optimisation using these reduce configuration spaces can find better pipelines.





\textit{The case of the dataset \textit{amazon}:} The r30 configuration space has the lowest mean error rate 29.33 (Table \ref{tab:error_rate_all_methods}). The best pipeline structure is CustomReplaceMissingValues $\rightarrow$ Normalize $\rightarrow$ RandomSubset $\rightarrow$ NaiveBayesMultinomial $\rightarrow$ RandomSubSpace. Figure \ref{fig:ranking_predictors} shows that the ranking of \textit{RandomSubSpace} is 21 and \textit{NaiveBayesMultinominal} is 2 for the dataset \textit{amazon}. However, these two ML predictor components are not both selected into configuration spaces from k1 to k19. Therefore, using reduced configuration spaces with the oracle and landmarking settings is not effective as the optimisation of hyperparameters of fixed well-performing pipeline structure due to the meta-knowledge base is not accurate in this case, though the rankings of all landmarking and oracle settings are better than \textit{baseline}.




We see that \textit{O-k4} and \textit{O-k8} have the best average rankings and exhibit a critical difference in comparison to the baseline configuration space, followed by \textit{L-k10}.
\textit{O-k4}, \textit{O-k8} and \textit{L-k10} are statistically different from the baseline configuration space.
The configuration space of \textit{L-k10} is reduced 67\% in comparison with the full configuration space.
Moreover, we see that the performance of SMAC decreases when increasing the value of \textit{k} in the oracle settings (\textit{O-k4} $>$ \textit{O-k8} $>$ \textit{O-k10} $>$ \textit{O-k19}). 
The reason is that the small \textit{k} value allows for generating small configuration spaces. Additionally, the best-performing components are always selected into the configuration spaces. Therefore, SMAC can spend more time on optimising hyperparameters to find better pipelines.
However, the results from the relative landmarking are different (\textit{L-k10} $>$ \textit{L-k8} $>$ \textit{L-k4} $>$ \textit{L-k19}).  
The average ranking of \textit{L-k10} is lower than \textit{O-k4} and \textit{O-k8}. The average ranking of \textit{L-k8}, \textit{L-k4}, \textit{L-k19} are lower than \textit{O-k19}. 
If the landmarking was able to recommend well-performing components to generate configuration spaces which are the same to the oracle configuration spaces, the performance of SMAC should be the same in both ways (e.g., \textit{L-k4} could be similar to \textit{O-k4})
Note that the meta-knowledge base which is extracted from the prior evaluations does not meet an extreme level of reliability which requires thorough evaluations of all ML components on many datasets that have diverse characteristics.
Therefore, the landmarking method may not select the best-performing ML components to generate configuration spaces with k=4 and k=8. Due to the uncertainty of the meta-knowledge base as well as the problem matching method (i.e., the landmarking method), a larger value of k should be selected to guarantee that the best-performing ML components are always chosen (i.e., \textit{L-k10} is better than \textit{L-k8} and  \textit{L-k8} is better than \textit{L-k4}). 
It suggests that the landmarking method, which is used to find the most similar prior problem, can be improved in future to enable the higher reduction of configuration spaces as the oracle settings.    
Although using \textit{L-k19} is slightly better than the baseline configuration space, \textit{L-k19} has a lower performance in comparison with \textit{L-k10}, \textit{L-k8} and \textit{L-k4}. This shows that if two configuration spaces both consist of the best-performing components, SMAC has a better performance using the smaller configuration space. 


%This set of experiments show that this meta-knowledge base is useful to reduce configuration spaces by selecting top 10 well-performing predictors of the most similar datasets (\textit{L-k10}). The configuration space of \textit{L-k10} is reduced 67\% in comparison with the full configuration space. In general, using the reduced configuration space of \textit{L-k10}, SMAC finds better well-performing pipelines than the ones with full configuration space. 

%For the dataset \textit{gisette}, we see that the \textit{O-k1} has the highest number of cases that have the best pipelines among configuration spaces (i.e., 5 cases of \textit{kddcup}, \textit{madelon}, \textit{shuttle}, \textit{winequality}, and \textit{yeast}), whereas O-k19 has the lowest (i.e., 1 case of \textit{kddcup}) (Table \ref{tab:error_rate_all_methods}). 

%Moreover, the best pipelines of all oracle settings are constructed by \textit{VotedPerceptron}. This indicates that if the configuration space is small and includes the top predictors, the ML pipeline composition and optimisation can dedicate time on hyperparameter optimisation to find better pipelines.

%\textit{The case of the dataset \textit{convex}:} In the case of using the fixed pipeline from the 30-hour optimisation (r30), the best pipeline structure is \textit{RandomForest} $\rightarrow$ \textit{AdaBoostM1}. The best pipeline structure of the other settings has only one component. L-k10 and O-k8 have the lowest mean error rate (i.e., 25.65 and 25.51). The best pipelines of L-k10 and O-k8 are \textit{RandomForest} and \textit{SMO} respectively. It shows that a complex pipeline which has more hyperparameters than a simple pipeline converges slower.

%\textit{The case of the dataset \textit{amazon}:} The r30 configuration space has the lowest mean error rate 29.33 (Table \ref{tab:error_rate_all_methods}). The best pipeline structure is CustomReplaceMissingValues $\rightarrow$ Normalize $\rightarrow$ RandomSubset $\rightarrow$ NaiveBayesMultinomial $\rightarrow$ RandomSubSpace. An interesting thing is that the ranking of \textit{RandomSubSpace} is 21 and \textit{NaiveBayesMultinominal} is 2. It shows that the pipelines have the lowest mean error rate may not contain the top 1 predictor. Therefore, selecting a values of k4, k8 and k10 can construct a better configuration spaces.


==> backup (210112)/6.conclusion.tex <==

\section{Conclusion}
\label{sec:conclusion}

In this study, we empirically demonstrate the efficiency of the use of the relative landmarking to reduce configuration spaces under the uncertainty of the meta-knowledge base which is generated from prior evaluations of ML pipeline composition and optimisation tasks. We show that the reasonable value of \textit{k} is 10 which is equivalent to one-third of the full configuration space. This value of \textit{k} depends on the factors including the reliability of the prior evaluations, the set of landmarkers as well as the similarity matching method that we use.
In future, we will extend this study to dynamically reduce configuration spaces based on the level of similarity between the new dataset and prior datasets.
If the similarity between the new dataset and prior datasets does not meet a certain threshold, we should reduce a small fraction of configuration spaces or even use full configuration spaces to guarantee the selection of well-performing ML components into the configuration space. If the similarity is high, we can reduce configuration spaces significantly to save time for hyperparameter optimisation.

%However, the quality of the meta-knowledge, the selection of the landmarkers, and the similarity matching method play crucial roles in the relative landmarking. Moreover, the evaluation time of the ML components and the landmakers is also another factor that can potentially be added into the meta-knowledge.
%It leads to a research challenge to improve the current relative landmarking method to have similar performance as the oracle settings by improving the above factors.





==> backup (210115)/0.abstract.tex <==
\begin{abstract}


Machine learning (ML) pipeline composition and optimisation have been studied to seek multi-stage ML models, i.e. preprocessor-inclusive, that are both valid and well-performing.
These processes typically require the design and traversal of complex configuration spaces consisting of not just individual ML components and their hyperparameters, but also higher-level pipeline structures that link these components together. 
Optimisation efficiency and resulting ML-model accuracy both suffer if this pipeline search space is unwieldy and excessively large; it becomes an appealing notion to avoid costly evaluations of poorly performing ML components ahead of time.
%The key research question then is whether this is both possible and effective by leveraging previous experience.
Accordingly, this paper investigates whether, based on previous experience, a pool of available classifiers/regressors can be preemptively culled ahead of initiating a pipeline composition/optimisation process for a new ML problem, i.e. dataset.
The previous experience comes in the form of classifier/regressor accuracy rankings derived, with loose assumptions, from a substantial but non-exhaustive number of pipeline evaluations; this meta-knowledge is considered `opportunistic'.
Numerous experiments with the AutoWeka4MCPS package, including ones leveraging similarities between datasets via the relative landmarking method, show that, despite its seeming unreliability, opportunistic meta-knowledge can improve ML outcomes.
However, results also indicate that the culling of classifiers/regressors should not be too severe either. In effect, it is better to search through a `top tier' of recommended predictors than to pin hopes onto one previously supreme performer.
% Several experiments are run,based on their performance rankings  ahead of the impact of configuration space reduction using the relative landmarking method. taking into account and considering a certain level of reliability of the meta-knowledge base generated from prior evaluations. To design a configuration space for a new problem, the top \textit{k} well-performing ML components of the most similar previously solved problem are used to design the configuration space for the new problem.
% %The experiments show the effectiveness of the relative landmarking method in reducing configuration spaces by selecting a reasonable value of \textit{k}.
% The experiments show that the most reasonable value of \textit{k} is 10 that is equivalent to the reduction of the full configuration space by 67\%. Moreover, the extreme value of \textit{k}=1 does not construct well-performing configuration spaces due to the uncertainty of the meta-knowledge base.









\end{abstract}

==> backup (210115)/1.introduction.tex <==

\section{Introduction}
\label{sec:intro}


Various ML pipeline composition and optimisation methods have been proposed in recent years to construct valid and well-performing multi-stage ML models, given both a problem (i.e., a dataset) and a set of ML components with tunable hyperparameters \cite{sabu18,zohu19,ngma20,kemu20}. Typically, this pool of ML components contains classification/regression predictors and other preprocessing operators, e.g. for imputation or feature generation/selection.
Among ML pipeline composition and optimisation methods, one of the most successful is based on the Sequential Model-based Algorithm Configuration (SMAC) approach \cite{thhu13}. Like most optimisers, this method seeks a balance between the exploration and exploitation of configuration spaces. When exploiting, the procedure investigates ML pipelines that are similar to the current best performers in terms of pipeline structure and hyperparameter values. When exploring, the procedure selects random candidates within configuration space instead, seeking to avoid entrapment in any local optima.

There are several automated machine learning (AutoML) tools that implement SMAC, starting with AutoWeka version 0.5 \cite{thhu13}. Most of these seek one-component pipelines and thus search through configuration spaces that only involve predictors and their hyperparameters. AutoWeka4MCPS is a rare exception, both extending configuration spaces for data preprocessing components and upgrading the implementation of SMAC, thus enabling the construction and optimisation of multiple-component pipelines \cite{sabu18}.
While this extension of configuration space allows a wider range of diverse and possibly better ML solutions to be explored, it does come with a number of challenges.
Key among them is that a large configuration space is more difficult to efficiently traverse for any optimiser. Given that every candidate ML pipeline must also be trained/queried on a dataset to evaluate its accuracy, and that training can be computationally expensive, this can be a substantial obstacle for using AutoML on a novel ML problem.
There is therefore both a need for and a great interest in approaches that offer the intelligent reduction of configuration spaces by preemptively excluding unpromising ML pipelines or, more severely, ML components. %Such a reduction has a crucial advantage of allowing the ML pipeline composition and optimisation methods to work in and explore smaller configuration spaces which are constructed from the most suitable and well-performing ML components.

Two approaches summarise the several attempts that have been made to deal with the problem of configuration space reduction: predefined pipeline structures and meta-learning. The former restricts ML-component composition to fixed structures \cite{sabu18,fekl15} or ad-hoc specifications \cite{depi17,tsga12,olmo16,wemo18,giya18} (e.g., context-free grammars) that leverage expert knowledge. This method for controlling pipeline structure is direct and relatively simple. However, the obvious drawback arises from the potential bias of expert knowledge, which may suppress the opportunity to find better ML solutions residing outside of predefined templates.
The major alternative approach is to employ meta-learning, with the aim of reducing configuration spaces by learning from prior evaluations. Some previous attempts under this banner have sought to cull search spaces by preemptively identifying ML components that perform the best \cite{dbbr18,va19,lebu15,albu15}, while others have focussed on important hyperparameters and appropriate value ranges for a given problem \cite{albu15,rihu18,prbo19,wemu20}. The studies in this latter case faced computational challenges, only investigating hyperparameters for up to six algorithms.% \cite{rihu18,prbo19,wemu20}.

In general, assembling a reliable meta-knowledge base is very difficult. Ideally, the construction of one should involve intensive evaluations of many ML components, each one thoroughly sampled across a frequently multi-dimensional range of hyperparameter values. To make matters more complicated, the performance of ML components can vary substantially between two intrinsically dissimilar datasets, and it is not even clear what kind of dataset characteristics should be a metric for that dissimilarity \cite{lega10,lega10a,albu15}.
%diverse characteristics \cite{lega10,lega10a,albu15}. 
%Therefore, generating a very reliable meta-knowledge base from prior evaluations is very difficult.
In practice, data scientists do not have access to a tailor-made meta-knowledge base. On the other hand, in the natural course of executing AutoML pipeline composition/optimisation processes on a dataset, data scientists do implicitly acquire accuracy evaluations for numerous ML-pipeline candidates. So, we ask the question: are these evaluations opportunistically useful? Can they recommend
%On account of the fact that we usually have prior evaluations resulting from executing automated ML pipeline composition and optimisation methods, we would like to address the research questions about 
how many and which ML components we should select when designing an ML-pipeline search space? 
%configuration spaces acknowledging and taking into account a certain level of accuracy and reliability of a meta-knowledge base generated from such prior evaluations.

To explore these research questions, we run a series of experiments with the AutoWeka4MCPS package \cite{sabu18}, which is accelerated by the ML-pipeline validity checker, AVATAR \cite{ngga20}, wherever specified. 
To accumulate `previous experience', we initially apply SMAC-based AutoML to 20 datasets, spending two hours for each, and extract a collection of ML-pipeline evaluations from the iterations of the SMAC optimisations. We then make a very loose approximation that, in the absence of further information, the error of a pipeline represents a sampled error of its constituent predictor, thus enabling the compilation of mean-error statistics for 30 Weka predictors, both overall and per dataset. The assumption involved in this process is of course contentious, but a key question is whether rankings from the compiled statistics are still reliable enough to at least guide an improved search for an ML solution to a new dataset.

Additionally, elements of our study attempt to improve upon general meta-knowledge by prioritising rankings from similar datasets. We employ the relative landmarking method \cite{va19} to quantify that similarity. Specifically, a newly encountered dataset is marked by a set of performance values, which are derived after executing a certain number of easy-to-evaluate landmarkers (i.e., single-component pipelines) on that dataset. These values are then correlated with the performance of those same landmarking predictors on previously encountered datasets; these error values are extracted from the compilation statistics in the meta-knowledge base.
%to reduce configuration spaces. We construct a meta-knowledge base from prior evaluations of two-hour ML pipeline composition and optimisation of SMAC over 20 datasets. The meta-knowledge base contains the mean error rate of ML components for each prior dataset.   
%The new dataset is evaluated by executing a certain number of landmarkers (i.e., single-component pipelines). The performance of the landmarkers on the new dataset is correlated with the performance of these landmarkers on prior datasets from the meta-knowledge base. The top \textit{k} well-performing ML components of the most similar dataset are selected to construct configuration spaces.

Ultimately, this study has two main contributions:

\begin{itemize}
    \item A definition of the problem of ML pipeline composition and optimisation with dynamic configuration spaces.
    
    \item An investigation of the performance impact on an AutoML composition/optimisation process by varying levels of pipeline search space reduction, i.e. removing all but the `best' $k$ of 30 predictors from an ML-component pool, for variable $k$. In particular, the focus of this study is on the `best' being defined by predictor rankings for the most similar dataset, as derived from opportunistic and somewhat unreliable meta-knowledge. %of the levels of the configuration space reduction (i.e., specified by different values of \textit{k}) on the performance of ML pipeline composition and optimisation methods given a certain level of reliability of the meta-knowledge base.
    
    
\end{itemize}




This paper is divided into 6 sections. After the Introduction,
Section \ref{sec:related_work} presents previous studies to reduce configuration spaces in the context of AutoML.
Section \ref{sec:search_space_modelling} formalises the problem definition of ML pipeline composition and optimisation with dynamic configuration spaces.
Section \ref{sec:relative_landmarking} presents the methodology of relative landmarking and its proposed use in reducing configuration spaces.
Section \ref{sec:experiment} presents experiments to investigate the problem of configuration space reduction. Finally, Section \ref{sec:conclusion} concludes this study.
 


==> backup (210115)/2.related_work.tex <==
\section{Related Work}
\label{sec:related_work}


The growing number of available ML methods with their often complex hyperparameters leads to a very rapid expansion, if not combinatorial explosion, of ML-pipeline configurations and associated search spaces. Intelligent reduction of these configuration spaces enables ML pipeline composition and optimisation methods to find valid and well-performing ML pipelines faster within the typical constraints of execution environments and time budgets.
We review two main approaches to reduce configuration spaces in the context of ML pipeline composition and optimisation. 

\textit{Predefined ML pipeline structures and component hyperparameters:} This approach can be implemented as fixed pipeline templates \cite{sabu18,fekl15} or ad-hoc specifications \cite{depi17,tsga12,olmo16,wemo18,giya18} such as context-free grammars. Moreover, specific ranges of hyperparameter values, which highly contribute to well-performing pipelines, are also predefined in these specifications.
The advantage of this approach is its simple nature, leveraging expert knowledge to reduce configuration spaces by directly restricting the length of ML pipelines, the pool of ML components, and their permissible orderings/arrangements. However, the disadvantage of this approach is that there might be strongly performing ML pipelines outside of the predefined templates. 


\textit{Meta-learning:} This approach aims to reduce configuration spaces by using prior knowledge to avoid wasting time with unpromising ML-solution candidates. Frequently, this involves assessing similarity between past and present ML problems/datasets, so as to hone in on the most relevant meta-knowledge available \cite{dbbr18,lebu15,lega10,albu15}. 
%learning the characteristics of prior evaluations. The main idea of this approach is to establish relationships between datasets' characteristics and the performance of ML components based on prior evaluations \cite{dbbr18,lebu15,lega10,albu15}.
To quantify this similarity, characteristics are typically established for datasets, which can then be used in correlations. A characteristic can be directly derived from the dataset as a meta-feature, e.g. the number of raw features or data instances. Alternatively, relevant to this study, two datasets can be compared by the relative performance of landmarkers. These landmarkers are ideally simple one-component pipelines, i.e. predictors, that are of varying types; they estimate the suitability of varying modelling approaches for a dataset. For instance, the performance of a linear regressor theoretically quantifies whether an ML problem is linear. An ML problem that is estimated to be nonlinear will likely not benefit from methods serving a linear dataset. In any case, the meta-learning approach can be used to reduce configuration spaces by selecting a number of well-performing ML components  \cite{albu15,dbbr18,va19,lebu15} or important hyperparameters for tuning \cite{albu15,rihu18,prbo19,wemu20}. For instance, both \textit{average ranking} and \textit{active testing} have previously been used to recommend ML solutions for new datasets \cite{dbbr18}. However, these approaches have not been applied to AutoML yet. Moreover, these studies limit their scopes by optimising predictors, not multi-component pipelines, and the optimisation method they use is grid search, proven not to be as effective as SMAC \cite{thhu13}. 
Other studies have investigated estimating the importance of hyperparameters \cite{rihu18,prbo19,wemu20} from prior evaluations. 
Specifically, some hyperparameters are more sensitive to perturbation than others; tuning them can contribute to a proportionally higher variability in ML-algorithm performance (i.e., error rate). As an example, gamma and complexity variable C are the most important hyperparameters for an SVM \cite{rihu18}.
Consequently, the results of these studies can be used to reduce configuration spaces by constraining less-important hyperparameters, either by making their search ranges less granular or outright fixing them as default values.  
This frees up more time to seek the best values for important hyperparameters that have the highest impact on finding well-performing pipelines.
However, a disadvantage of these studies is that the importance of ML-component hyperparameters has only been studied on small sets of up to six algorithms. This reflects how time-consuming it is to properly sample hyperparameter space across all available algorithms. 

In this study, our approach aligns with meta-learning principles. However, it differs from previous studies by refusing to carefully curate a tailor-made meta-knowledge base. Instead, accepting a degree of unreliability, we opportunistically derive assumptive statistics from numerous pipeline evaluations; these evaluations are non-exhaustive and simulate the remnants of AutoML optimisation processes intended to solve seemingly unrelated problems. %acknowledges and accepts a certain level of reliability of prior evaluations which are used to build a meta-knowledge base. 
Faced with this context, we focus on the relative landmarking method to draw similarities between past and present datasets, then we identify previously well-performing ML components, around which we constrain configuration subspaces for ML pipeline composition and optimisation. We also investigate how varying degrees of this recommendation-based search-space culling affects the performance of ML pipeline composition/optimisation methods.


==> backup (210115)/3.search_space_modeling.tex <==

\section{Modelling Configuration Spaces for ML Pipeline Composition and Optimisation }
\label{sec:search_space_modelling}

To control the extension and reduction of configuration spaces in the context of AutoML, we model them using a generic tree structure. After that, we extend the problem of pipeline composition and optimisation \cite{sabu18} by adding a factor representing pipeline structures. Finally, we define the problem of pipeline composition and optimisation with dynamic configuration spaces as a constrained optimisation problem.



\subsection{Configuration Space Modelling}

To discuss the search space of ML pipelines, it is worth considering that each potential constituent within a pipeline is an instantiation of an ML component with a certain set of values for its hyperparameters. Specifically, if $\mathcal{A}$ is the pool of available ML components, a potential pipeline constituent indexed by $c$ can be represented as
%Given a tree-structured set of nodes $\mathcal{X}$ and a set of ML components $\mathcal{A}$, for each tree node $x_i \in \mathcal{X}$:
\begin{equation}
\small{
x_c=(\mathcal{A}_c,\lambda_c, \epsilon_c),
\label{eq:treenode}
}
\end{equation}
where $\mathcal{A}_c\in\mathcal{A}$ is an ML component and $\lambda_c$ is a set of hyperparameter values for component $\mathcal{A}_c$. Notably, we also mark the candidate by binary variable $\epsilon_c$, which represents whether the potential constituent is accessible/inaccessible to a pipeline search algorithm. %the active/inactive status of this node. If a node is a predictor and has the inactive status, all of its children node are recursively inactive.

We now arrange the set of candidate constituents, $\mathcal{X}=\{x_c\}$, in a tree-based configuration space defined as
\begin{equation}
\small{
\mathcal{T}=(\mathcal{X},f_p).
\label{eq:searchtree}
}
\end{equation}
Function $f_p$ represents the assignment of each node $x_c$ to a parent node $f_p(x_c)$, where the root nodes of this tree-structured space are defined by  $f_p(x_c)=x_c$. 

Given this space, an ML pipeline $p$, also called a configuration, is a path constructed by back tracking from an active leaf node to the root node. Specifically, 
\begin{equation}
\small{
p = (g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}}),
\label{eq:pipeline}
}
\end{equation}
where $\vec{\mathcal{A}}$ is a vector of ML components in $\mathcal{A}$, $\vec{\mathcal{\lambda}}$ is a vector of hyperparameter-value sets corresponding to $\vec{\mathcal{A}}$, and $g$ is a sequential pipeline structure that defines how the components are connected. 
Configuration space $\mathcal{T}$ can always be extended by adding tree nodes, but dynamically reducing pipeline search space to a subset of $\mathcal{T}$ is also possible by `deactivating' tree nodes, i.e. flipping their $\epsilon_c$ switches and those of any appropriate branches. Specifically, if a candidate pipeline contains a deactivated node, it is invalid and can be ignored by any search algorithm like SMAC \cite{thhu13}.




\subsection{The Problem of Pipeline Composition and Optimisation with Dynamic Configuration Spaces}


The aim of pipeline composition and optimisation is to find the best-performing ML pipeline $(g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{*}$, which involves the optimal combination of pipeline structure, selected components, and associated hyperparameters. The formalism of the pipeline-search problem \cite{sabu18} can thus be written as
\begin{equation}
\small{
(g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{*} = \mathrm{arg\,min}\frac{1}{k}\sum_{i=1}^{k} \mathcal{L}((g,\vec{\mathcal{A}},\vec{\mathcal{\lambda}})^{(i)},\mathcal{D}^{(i)}_{train},\mathcal{D}^{(i)}_{valid}),
}
\label{eq:pipeline_problem}
\end{equation}
where $\mathcal{D}_{train}$ and $\mathcal{D}_{valid}$ are training and validation datasets. Specifically, this equation minimises the k-fold cross validation error of loss function $\mathcal{L}$. The $k$ here is not to be confused with the $k$ variable used for predictor rankings elsewhere in this paper.




Equation (\ref{eq:pipeline_problem}) does not consider changes to the configuration space $\mathcal{T}$. If we reduce this configuration space by selecting promising pipelines to form the configuration subspace $\mathcal{T}^{*}\subset \mathcal{T}$, the problem of pipeline composition/optimisation can be reformulated as a constrained version of Eq. (\ref{eq:pipeline_problem}), as follows:  
\begin{equation}
\small{
(g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{*} = \mathrm{arg\,min}\frac{1}{k}\sum_{i=1}^{k} \mathcal{L}((g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{(i)} \in \mathcal{T}',\mathcal{D}^{(i)}_{train},\mathcal{D}^{(i)}_{valid})
}
\label{eq:extended_pipeline_problem}
\end{equation}
subject to
\begin{equation}
\small{
%\mathcal{T}^{*} \subset \mathcal{T} \:\:\:\:\:  \textit{and} \:\:\:\:\:  h(\mathcal{T}^{*}) = \emptyset,
\mathcal{T}' = \mathcal{T}^{*}\setminus h(\mathcal{T}^{*}),
\label{eq:extended_pipeline_problem_constraints_1}
}
\end{equation}
where $h(\mathcal{T}^{*})$ is an optional function to find the set of all invalid pipelines. This set exclusion can be considered to represent the role of AVATAR \cite{ngga20}.




==> backup (210115)/4.relative_landmarking.tex <==

\section{Configuration Space Reduction Using the Relative Landmarking Method}
\label{sec:relative_landmarking}

In this section, we present the methodology to design configuration spaces for the ML pipeline composition and optimisation given the meta-knowledge base of uneven quality and certain level of uncertainty. A relative landmarking method, inspired by the \textit{average ranking} \cite{dbbr18} and the \textit{relative landmarking} \cite{va19} approaches, is proposed. These methods are used to recommend an ML algorithm for a given dataset though they have not considered the optimisation time budget or have been proposed in the context of the automated composition and optimisation of ML pipelines which are both the subject of our primary investigations. 
Besides, there exists an uncertainty in the meta-knowledge base, which describes the relationships between the average performance of ML components and the datasets' characteristics. 
This uncertainty is due to the lack of a thorough evaluation which covers the combined effects of ML components in pipelines, the diversity of pipeline structures and components' hyperparameters.
To be more specific, because the meta-knowledge base is generated from prior evaluations of the automated composition and optimisation, the number of times, that ML components are evaluated, is different. There are even those that have not been evaluated or have been evaluated with a small number of times due to the limit of the optimisation time budget.
Such thorough evaluations to generate highly reliable meta-knowledge are prohibitively expensive in the context of ML pipeline composition and optimisation task and we are interested in investigating if at all and how partial or less reliable meta-knowledge can be effectively used in our context.
    

Firstly, we present the problem formulation of configuration space reduction using the relative landmarking method. Secondly, we present landmarkers that are used to evaluate a new dataset to understand its characteristics. Thirdly, we present the algorithm to design configuration spaces given a new dataset and prior evaluations on other problems from which, we assume, a useful knowledge can be extracted.




\subsection{Problem Formulation}
\label{sec:problem_formulation}


We define the problem of pipeline composition and optimisation with dynamic configuration spaces in Equation \ref{eq:extended_pipeline_problem}. An optimal configuration space $\mathcal{T}^{*}$ can be designed at the initialisation of the ML pipeline composition and optimisation methods. The configuration space $\mathcal{T}^{*}$ of the new dataset is constructed by \textit{k} best performing ML components of the most similar dataset from prior evaluations.

Given a new dataset $t_{new}$, we need to find a prior dataset $t^{*}_{i}$ which is similar to $t_{new}$ \cite{va19}. In order to do that, we evaluate a set of landmarkers (i.e., pipelines) $\Theta=\{\theta_i\}$  on $t_{new}$ and record their performance results $E_{new}$. We measure the relative similarity of the performance of the landmarkers between the new dataset $t_{new}$ and the prior dataset $t_{i}$. We select the most similar dataset $t^{*}_{i}$ based on the ranking of the similarity. The configuration space  $\mathcal{T}_{new}$ of the dataset $t_{new}$ is constructed by selecting the top $k$ well-performing ML components of the previously tackled dataset $t^{*}_{i}$.



\subsection{Landmarkers}

Landmarkers \cite{va19} $\Theta=\{\theta_i\}$ are the ML methods/pipelines. They are usually simple and efficient to execute. 
They are used to indirectly evaluate the characteristics of datasets through  evaluations of their performance (e.g., classification accuracy) which can then be used as meta-features.
These meta-features are used to find the most similar previously solved dataset by matching the relative performance of the landmarkers on the new dataset and the previously solved datasets.
Selecting a set of landmarkers, or more generally a set of meta-features describing complex problems, obviously has an impact on the final results as shown in a number of previous studies on the subject \cite{va19,albu15}. As in the context of AutoML, the evaluation time of the landmarkers forms a part of the overall AutoML optimisation time, in this study we have made a deliberate decision to evaluate a limited set of landmarkers which are the fastest to execute. Therefore in our experiments we use the five fastest predictors (i.e., RandomTree, ZeroR, IBk, NaiveBayes and OneR) from the compiled ranking of the average evaluation time of the pipelines containing these components in prior evaluations. We acknowledge that this choice is not optimal in any other sense than their cumulative execution time but it is a part of our study goals whether such a crude approach for complex problems matching could still be effective, and to what extent, in reduction of our input search space for AutoML algorithms.



\subsection{Dynamic Configuration Space Design}



\begin{algorithm}[!htbp]
\small

\caption{\small Design Configuration Space Using The Relative Landmarking}
\begin{algorithmic}[1]
\Require
      \Statex $\Theta$: The set of landmarkers
      \Statex $t_{new}$: The new dataset
      \Statex $t_{prior}$: The prior dataset
\Statex      
\For{$\theta_i$ \textbf{in}  $\Theta$}
        \State $E_{new}\_i$ = \textit{evaluate}($\theta_i$, $t_{new}$)
\EndFor
\For{\textbf{each}  $t_{prior}\_i$}
        \State $correlation\_coefficient_i$ = 
        
        \textit{calculateCorrelation}($E_{new}$, $E_{prior}\_i$)
\EndFor
\State $t^{*}$ = \textit{getMostSimilarTask}($correlation\_coefficient$) 
\State $\mathcal{T}_{new}$ = \textit{selectMLComponents}($t^{*}$, $k$)
\State \textbf{return} $\mathcal{T}_{new}$
\end{algorithmic}
\label{algorithm:construct_configuration_space}
\end{algorithm} 




Algorithm \ref{algorithm:construct_configuration_space} presents the algorithm to design a configuration space using the relative landmarking method. This configuration space is used as an input for AutoML pipeline composition and optimisation methods. Firstly, the algorithm evaluates the new dataset $t_{new}$ using each landmarker $\theta_i$. The result is the performance $E_{new}\_i$ (e.g., the 10-fold cross-validation error rate) of this landmarker (line 1-3). Secondly, the algorithm calculates Pearson correlation coefficient of $E_{new}\_i$ with the mean error rate of the landmarkers on previously solved datasets $E_{prior}\_i$ (line 4-6). Thirdly, the algorithm ranks the correlation coefficients and selects the dataset $t^{*}$ that has the highest correlation coefficient (line 7). Finally, the configuration space is constructed by all preprocessing components and top \textit{k} best performing predictors (line 8) of the most similar dataset $t^{*}$. Note that sum of the evaluation time of landmarkers on the new dataset is deducted from the total time budget of the ML pipeline composition and optimisation task.

==> backup (210115)/5.experiments.tex <==
\section{Experiments}
\label{sec:experiment}

In the experiments, we use the method described in Section \ref{sec:relative_landmarking} to explore the impact of the levels of configuration space reduction on the performance of AutoML composition and optimisation method. 
To do so, we compare the mean error rate of five approaches to design the configuration spaces:

\begin{itemize}
    \item \textbf{baseline}: The full configuration space as is constructed by the preprocessing and predictor components that are implemented in AutoWeka4MCPS \cite{sabu18}. The reduction of configuration spaces is effective only if this reduction enables SMAC to find better pipelines than using the baseline configuration space.
    
    \item \textbf{r30}: A restricted configuration space using fixed pipeline structures extracted from the best pipelines found within 30 hours optimisation time \cite{sabu18}. By using this configuration space, the AutoML composition and optimisation method dedicates time to optimise hyperparameters of the fixed ML pipelines. We use this configuration to illustrate the trade-off between only optimising hyperparameters of fixed complex pipelines and searching for both well-performing pipeline structures and their hyperparameters within the reduced configuration spaces.
    
    
    \item \textbf{avatar}: The full configuration space which is similar to the \textbf{baseline} configuration space, but we use the AVATAR\cite{ngma20} to reduce configuration spaces by quickly ignoring invalid pipelines when using SMAC to exploit and explore the baseline configuration space. 
    
    
    \item \textbf{oracle settings (\textit{O-k1}, \textit{O-k4}, \textit{O-k8}, \textit{O-k10}, and \textit{O-k19})}: The oracle configuration spaces designed by selecting k (i.e., k in $\{1,4,8,10,19\}$) predictors which have the lowest mean error rate in prior evaluations for the datasets themselves.
    The purpose of using oracle settings is to demonstrate that even if we ignore the impact of using the landmarking method to find the most similar prior problem, the meta-knowledge base which is generated from prior evaluations of AutoML composition and optimisation is useful and meet a certain level of reliability to be used for the reduction of configuration spaces.
    
    
    
    
    \item \textbf{landmarking settings (\textit{L-k1}, \textit{L-k4}, \textit{L-k8}, \textit{L-k10}, and \textit{L-k19})}: The relative landmarking configuration spaces designed by selecting k (i.e., k in $\{1,4,8,10,19\}$) predictors which have the lowest mean error rate in prior evaluations of the most similar dataset using the relative landmarking. We use the landmarking settings for the experiment to show that how much should we reduce configuration spaces if there exists uncertainties of both the meta-knowledge base and the matching method (i.e., the landmarking method) we use the find the most similar prior problems.
    
    
    
    
\end{itemize}


\subsection{Experimental settings}

For the experiments we will use a variety of datasets which are presented in Table \ref{tab:datasets}.
The AutoML tool we use for the experiments is AutoWeka4MCPS\footnote{https://github.com/UTS-AAi/autoweka} which implements the method of configuration space reduction using the relative landmarking.
The ML pipeline composition and optimisation method is SMAC. 
We also use the AVATAR to evaluate the validity of ML pipelines \cite{ngga20} which dynamically reduces configuration spaces by ignoring invalid pipelines which are generated during the exploration and exploitation of SMAC.
We set the time budget to 2 hours and the memory to 1GB.
We perform five runs of experiment for each dataset and report the mean error rate of the best pipelines found.  
We use the leave-one-out strategy for the experiments with regard to the meta-data availability.
For each dataset, we exclude the prior evaluations of this dataset from the meta-knowledge base when performing the relative landmarking method to reduce configuration spaces. The optimisation time for SMAC in cases of using the relative landmarking method is the remaining time of 2 hours after using the landmarking method to construct the configuration spaces. 

We have conducted a preliminary study to investigate the feasibility of configuration space reduction using the relative landmarking method  by extracting prior evaluations. We use Algorithm \ref{algorithm:construct_configuration_space} to design configuration spaces for each dataset.
We extract the prior evaluations of the most similar dataset found using the relative landmarking method. The extracted evaluations exclude pipelines that are not in the reduced configuration spaces. We make an assumption that these extracted evaluations are the results of the ML pipeline composition and optimisation without running the optimisation tasks that are time-consuming.
By doing so, we have to accept an issue that the total optimisation time of the extracted evaluations is less than total budget time (i.e., 2h). However, we can quickly select a subset of \textit{k} which is used to perform both the configuration space reduction as well as the pipeline composition and optimisation with the reduced configuration spaces.
For each dataset, we compare the ranking of predictors of different reduced configuration spaces \textit{k-space} and the configuration space constructed by selecting the top 8 well-performing predictor components of all datasets (\textit{avg-k8}).
The size of \textit{avg-k8} is approximately 25\% of the full configuration space.
We select 8 components for this exploratory study because we expect the landmarking method is effective when it comes to constructing a configuration space consisting of ML components which are better than the top 25\% average well-performing components from all prior evaluations.


Figure \ref{fig:k_Values} shows the number of cases (i.e., datasets) with the ranking of the best ML component in \textit{k-space} is higher than or equal the one in \textit{avg-k8} (metric-k). We can see that \textit{metric-k} increases when the value of \textit{k} increases because of the increase of the possibility for the best ML component being among the \textit{k} selected components. We choose 5 values of \textit{k} (i.e., 1, 4, 8, 10 and 19) to generate the configuration spaces and run the ML pipeline composition and optimisation tasks using these configuration spaces. We choose these values of \textit{k} because of the following reasons:

\begin{itemize}
    \item The value of k=1 is with the minimum configuration space.
    \item The values of k from 19 to 30 have the same \textit{metric-k}. The values of k from 10 to 18 also have the same \textit{metric-k}. We choose the smallest value of k=19 and k=10 because we want to maximise the reduction of configuration spaces.
    \item The values of k=4 and k=8 were chosen as they are between k=1 and k=10 so offer the best coverage of the space.
\end{itemize}




%\vspace{-0.60cm}
\begin{figure*}[htbp]
\centering
\includegraphics[width=0.95\linewidth]{images/exp1_k_values.pdf}
\caption{The number of cases (i.e., datasets) with the ranking of the best ML component in \textit{k-space} is higher than or equal the one in \textit{avg-k8} (metric-k).}
\label{fig:k_Values}
\end{figure*}


\input{tables/tab_dataset}
%\include{tables/tab_histotical_runs_predictors_and_ranking_mean_error}



%\subsection{Investigate the impact of selecting different values of k of the relative landmarking}

\subsection{Experiment Results}


%move to supplementary documents
\input{tables/tab_error_all_methods}
\input{tables/tab_pipelines_apart}

%\include{tables/tab_pipelines_1}
%\include{tables/tab_error_all_methods_ranking}
%\input{tables/tab_pipelines_2}
%\include{tables/tab_pipelines_3}




%\input{tables/tab_landmarking_results_extractedhistory}



%To facilitate the study, we use prior evaluations of AutoWeka4MCPS with 2 hours optimisation time, 1GB memory, using SMAC as the ML pipeline composition and optimisation method over 20 datasets. 
%We extracts the mean error rate of predictors based on the error rate of their ML pipelines within 20 datasets in the prior evaluations. Based on the mean error rate of the predictors, we generate the ranking of predictors across 20 datasets, as shown in Figure \ref{fig:ranking_predictors}. We can see that there is no predictor has the best ranking across all datasets. For example, the component \textit{Logistic} has the top ranking in the cases of the datasets \textit{abalone}, \textit{semeion} and \textit{waveform}. However, this component ranks 19\textsuperscript{th} and 26\textsuperscript{th} in the case of the datasets \textit{convex} and \textit{secom}.



Table \ref{tab:error_rate_all_methods} presents the mean error rate (\%) of the best pipelines found by SMAC using different methods to design configuration spaces.
The lowest mean error rate for each dataset is shown in bold. The `-' symbol represents a ``not found'' solution due to incomplete runs within the optimisation time. Figure \ref{fig:cd_diagram} shows the critical difference diagram of the average rankings of the mean error rate with different configuration spaces.
Table \ref{tab:pipelines}\footnote{The details of the best ML pipelines found by SMAC with different configuration spaces for all data sets can be found at \url{https://github.com/UTS-AAi/autoweka/blob/master/autoweka4mcps/doc/landmarking_supplementary.pdf} } shows the best ML pipelines found by SMAC with different configuration spaces for the data sets \textit{amazon} and \textit{convex}. .


\begin{figure}[h] 
    \centering
    \includegraphics[width=0.8\linewidth]{images/cd_all_methods.pdf}
    \caption{The critical difference diagram of the average ranking of the performance of SMAC with different configuration spaces.}
    \label{fig:cd_diagram}
\end{figure}

\begin{figure}[h] 
\includegraphics[width=1.00\linewidth]{images/mlcomponent_ranking_part.pdf}
\caption{The ranking of ML predictor components based on mean error rate of their pipelines from prior evaluations for selected datasets.}
\label{fig:ranking_predictors}
\end{figure}


\textit{Extreme values of \textit{k}=1 and k=19:} We can see that the values of \textit{k} that resulted in the worst performance is 1 and 19 in both cases of the relative landmarking and the oracle. We can also see that when selecting \textit{k} equals 1 (i.e., \textit{L-k1} and \textit{O-k1}), SMAC finds pipelines that have the lowest error rate of 5 in 20 datasets that is higher than using other configuration spaces.
Moreover, the number of incomplete optimisation tasks of \textit{L-k1} and \textit{O-k1} is 5 and 4 respectively that is also higher than the other methods. The reason is that the selection of the extreme value of \textit{k}=1 can reduce the configuration spaces significantly. If the relative landmarking method can recommend a well-performing predictor component accurately, SMAC can spend more time for the hyperparameter optimisation of pipelines containing this ML component. 
Therefore, the extreme selections of k1 have more chance to find the well-performing pipelines. However, SMAC does not have an opportunity to explore other solutions in cases the selected predictor component, which is recommended by the relative landmarking, is not well-performing due to the lack of thorough evaluations of this component. For example, for the dataset \textit{amazon}, \textit{L-k1} has the highest error rate which has the configuration space constructed from \textit{Logistic}. However, the pipeline that has the minimum mean error rate is a pipeline containing \textit{NaiveBayesMultinominal}. We also see that for the datasets \textit{abalone, adult, car, dexter} and \textit{waveform}, \textit{L-k1} has the lowest mean error rate although the average ranking \textit{L-k1} is only better than the cases using the full configuration space (i.e., \textit{baseline}). 
The selection of k19 makes its configuration space to be larger than ones of k1, k4, k8 and k10. Therefore, SMAC has less time for the hyperparameter optimisation. It is even worsen than using the full configuration spaces if the top predictors are not selected into the configuration spaces due to the uncertainty of the meta-knowledge base. The average ranking of \textit{L-k19} is slightly better than \textit{L-k1} and \textit{baseline}, 8.25 compared with 8.80 and 9.65 (Figure \ref{fig:cd_diagram}).


\textit{The middle values of k=4, k=8 and k=10}: The selection of k4, k8 and k10 can construct a better configuration spaces than the extreme values k1 and k19. It can avoid the extreme selection of only one predictor component which may not be well-performing, as well as the design of large configuration spaces which are difficult to be explored within a time budget.
Figure \ref{fig:cd_diagram} shows that \textit{L-k10} is critically different from the \textit{baseline} configuration space, 5.50 compared with 9.56. In other words, the relative landmarking with k10 can effectively reduce the configuration spaces to enable the ML composition and optimisation method to find better pipelines. 



\textit{The case of the dataset \textit{convex}:} In the case of using the fixed pipeline from the 30-hour optimisation (r30), the best pipeline structure is \textit{RandomForest} $\rightarrow$ \textit{AdaBoostM1} having the mean error rate 18.47 that is reported from the study of Savaldor et al. \cite{sabu18}. However, our experiment shows that the mean error rate of using \textit{r30} with 2-hour optimisation in case of \textit{convex} is 46.72.  
The best pipeline structure of the other settings has only one component. L-k10 and O-k8 have the lowest mean error rate (i.e., 25.65 and 25.51). The best pipelines of L-k10 and O-k8 are \textit{RandomForest} and \textit{SMO} respectively. It clearly shows that performing hyperparameter optimisation for a complex pipeline may not produce a well-performing pipeline in comparison with performing AutoML composition and optimisation using reduce configuration spaces (i.e., in the cases of O-k1, O-k4, O-k8, O-k10, O-k19, L-k8 and L-k10). 
The reason is that it takes more time to optimise hyperparameters of a complex pipeline and the given time budget is not enough. In these cases, performing AutoML composition and optimisation using these reduce configuration spaces can find better pipelines.





\textit{The case of the dataset \textit{amazon}:} The r30 configuration space has the lowest mean error rate 29.33 (Table \ref{tab:error_rate_all_methods}). The best pipeline structure is CustomReplaceMissingValues $\rightarrow$ Normalize $\rightarrow$ RandomSubset $\rightarrow$ NaiveBayesMultinomial $\rightarrow$ RandomSubSpace. Figure \ref{fig:ranking_predictors} shows that the ranking of \textit{RandomSubSpace} is 21 and \textit{NaiveBayesMultinominal} is 2 for the dataset \textit{amazon}. However, these two ML predictor components are not both selected into configuration spaces from k1 to k19. Therefore, using reduced configuration spaces with the oracle and landmarking settings is not effective as the optimisation of hyperparameters of fixed well-performing pipeline structure due to the meta-knowledge base is not accurate in this case, though the rankings of all landmarking and oracle settings are better than \textit{baseline}.




We see that \textit{O-k4} and \textit{O-k8} have the best average rankings and exhibit a critical difference in comparison to the baseline configuration space, followed by \textit{L-k10}.
\textit{O-k4}, \textit{O-k8} and \textit{L-k10} are statistically different from the baseline configuration space.
The configuration space of \textit{L-k10} is reduced 67\% in comparison with the full configuration space.
Moreover, we see that the performance of SMAC decreases when increasing the value of \textit{k} in the oracle settings (\textit{O-k4} $>$ \textit{O-k8} $>$ \textit{O-k10} $>$ \textit{O-k19}). 
The reason is that the small \textit{k} value allows for generating small configuration spaces. Additionally, the best-performing components are always selected into the configuration spaces. Therefore, SMAC can spend more time on optimising hyperparameters to find better pipelines.
However, the results from the relative landmarking are different (\textit{L-k10} $>$ \textit{L-k8} $>$ \textit{L-k4} $>$ \textit{L-k19}).  
The average ranking of \textit{L-k10} is lower than \textit{O-k4} and \textit{O-k8}. The average ranking of \textit{L-k8}, \textit{L-k4}, \textit{L-k19} are lower than \textit{O-k19}. 
If the landmarking was able to recommend well-performing components to generate configuration spaces which are the same to the oracle configuration spaces, the performance of SMAC should be the same in both ways (e.g., \textit{L-k4} could be similar to \textit{O-k4})
Note that the meta-knowledge base which is extracted from the prior evaluations does not meet an extreme level of reliability which requires thorough evaluations of all ML components on many datasets that have diverse characteristics.
Therefore, the landmarking method may not select the best-performing ML components to generate configuration spaces with k=4 and k=8. Due to the uncertainty of the meta-knowledge base as well as the problem matching method (i.e., the landmarking method), a larger value of k should be selected to guarantee that the best-performing ML components are always chosen (i.e., \textit{L-k10} is better than \textit{L-k8} and  \textit{L-k8} is better than \textit{L-k4}). 
It suggests that the landmarking method, which is used to find the most similar prior problem, can be improved in future to enable the higher reduction of configuration spaces as the oracle settings.    
Although using \textit{L-k19} is slightly better than the baseline configuration space, \textit{L-k19} has a lower performance in comparison with \textit{L-k10}, \textit{L-k8} and \textit{L-k4}. This shows that if two configuration spaces both consist of the best-performing components, SMAC has a better performance using the smaller configuration space. 


%This set of experiments show that this meta-knowledge base is useful to reduce configuration spaces by selecting top 10 well-performing predictors of the most similar datasets (\textit{L-k10}). The configuration space of \textit{L-k10} is reduced 67\% in comparison with the full configuration space. In general, using the reduced configuration space of \textit{L-k10}, SMAC finds better well-performing pipelines than the ones with full configuration space. 

%For the dataset \textit{gisette}, we see that the \textit{O-k1} has the highest number of cases that have the best pipelines among configuration spaces (i.e., 5 cases of \textit{kddcup}, \textit{madelon}, \textit{shuttle}, \textit{winequality}, and \textit{yeast}), whereas O-k19 has the lowest (i.e., 1 case of \textit{kddcup}) (Table \ref{tab:error_rate_all_methods}). 

%Moreover, the best pipelines of all oracle settings are constructed by \textit{VotedPerceptron}. This indicates that if the configuration space is small and includes the top predictors, the ML pipeline composition and optimisation can dedicate time on hyperparameter optimisation to find better pipelines.

%\textit{The case of the dataset \textit{convex}:} In the case of using the fixed pipeline from the 30-hour optimisation (r30), the best pipeline structure is \textit{RandomForest} $\rightarrow$ \textit{AdaBoostM1}. The best pipeline structure of the other settings has only one component. L-k10 and O-k8 have the lowest mean error rate (i.e., 25.65 and 25.51). The best pipelines of L-k10 and O-k8 are \textit{RandomForest} and \textit{SMO} respectively. It shows that a complex pipeline which has more hyperparameters than a simple pipeline converges slower.

%\textit{The case of the dataset \textit{amazon}:} The r30 configuration space has the lowest mean error rate 29.33 (Table \ref{tab:error_rate_all_methods}). The best pipeline structure is CustomReplaceMissingValues $\rightarrow$ Normalize $\rightarrow$ RandomSubset $\rightarrow$ NaiveBayesMultinomial $\rightarrow$ RandomSubSpace. An interesting thing is that the ranking of \textit{RandomSubSpace} is 21 and \textit{NaiveBayesMultinominal} is 2. It shows that the pipelines have the lowest mean error rate may not contain the top 1 predictor. Therefore, selecting a values of k4, k8 and k10 can construct a better configuration spaces.


==> backup (210115)/6.conclusion.tex <==

\section{Conclusion}
\label{sec:conclusion}

In this study, we empirically demonstrate the efficiency of the use of the relative landmarking to reduce configuration spaces under the uncertainty of the meta-knowledge base which is generated from prior evaluations of ML pipeline composition and optimisation tasks. We show that the reasonable value of \textit{k} is 10 which is equivalent to one-third of the full configuration space. This value of \textit{k} depends on the factors including the reliability of the prior evaluations, the set of landmarkers as well as the similarity matching method that we use.
In future, we will extend this study to dynamically reduce configuration spaces based on the level of similarity between the new dataset and prior datasets.
If the similarity between the new dataset and prior datasets does not meet a certain threshold, we should reduce a small fraction of configuration spaces or even use full configuration spaces to guarantee the selection of well-performing ML components into the configuration space. If the similarity is high, we can reduce configuration spaces significantly to save time for hyperparameter optimisation.

%However, the quality of the meta-knowledge, the selection of the landmarkers, and the similarity matching method play crucial roles in the relative landmarking. Moreover, the evaluation time of the ML components and the landmakers is also another factor that can potentially be added into the meta-knowledge.
%It leads to a research challenge to improve the current relative landmarking method to have similar performance as the oracle settings by improving the above factors.





==> sections/3.search_space_modeling.tex <==

\section{Modelling Configuration Spaces for ML Pipeline Composition and Optimisation }
\label{sec:search_space_modelling}

To control the extension and reduction of configuration spaces in the context of AutoML, we model them using a generic tree structure. After that, we extend the problem of pipeline composition and optimisation \cite{sabu18} by adding a factor representing pipeline structures. Finally, we define the problem of pipeline composition and optimisation with dynamic configuration spaces as a constrained optimisation problem.



\subsection{Configuration Space Modelling}

To discuss the search space of ML pipelines, it is worth considering that each potential constituent within a pipeline is an instantiation of an ML component with a certain set of values for its hyperparameters. Specifically, if $\mathcal{A}$ is the pool of available ML components, a potential pipeline constituent indexed by $c$ can be represented as
%Given a tree-structured set of nodes $\mathcal{X}$ and a set of ML components $\mathcal{A}$, for each tree node $x_i \in \mathcal{X}$:
\begin{equation}
\small{
x_c=(\mathcal{A}_c,\lambda_c, \epsilon_c),
\label{eq:treenode}
}
\end{equation}
where $\mathcal{A}_c\in\mathcal{A}$ is an ML component and $\lambda_c$ is a set of hyperparameter values for component $\mathcal{A}_c$. Notably, we also mark the candidate by binary variable $\epsilon_c$, which represents whether the potential constituent is accessible/inaccessible to a pipeline search algorithm. %the active/inactive status of this node. If a node is a predictor and has the inactive status, all of its children node are recursively inactive.

We now arrange the set of candidate constituents, $\mathcal{X}=\{x_c\}$, in a tree-based configuration space defined as
\begin{equation}
\small{
\mathcal{T}=(\mathcal{X},f_p).
\label{eq:searchtree}
}
\end{equation}
Function $f_p$ represents the assignment of each node $x_c$ to a parent node $f_p(x_c)$, where the root nodes of this tree-structured space are defined by  $f_p(x_c)=x_c$. 

Given this space, an ML pipeline $p$, also called a configuration, is a path constructed by back tracking from an active leaf node to the root node. Specifically, 
\begin{equation}
\small{
p = (g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}}),
\label{eq:pipeline}
}
\end{equation}
where $\vec{\mathcal{A}}$ is a vector of ML components in $\mathcal{A}$, $\vec{\mathcal{\lambda}}$ is a vector of hyperparameter-value sets corresponding to $\vec{\mathcal{A}}$, and $g$ is a sequential pipeline structure that defines how the components are connected. 
Configuration space $\mathcal{T}$ can always be extended by adding tree nodes, but dynamically reducing pipeline search space to a subset of $\mathcal{T}$ is also possible by `deactivating' tree nodes, i.e. flipping their $\epsilon_c$ switches and those of any appropriate branches. Specifically, if a candidate pipeline contains a deactivated node, it is invalid and can be ignored by any search algorithm like SMAC \cite{thhu13}.




\subsection{The Problem of Pipeline Composition and Optimisation with Dynamic Configuration Spaces}


The aim of pipeline composition and optimisation is to find the best-performing ML pipeline $(g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{*}$, which involves the optimal combination of pipeline structure, selected components, and associated hyperparameters. The formalism of the pipeline-search problem \cite{sabu18} can thus be written as
\begin{equation}
\small{
(g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{*} = \mathrm{arg\,min}\frac{1}{k}\sum_{i=1}^{k} \mathcal{L}((g,\vec{\mathcal{A}},\vec{\mathcal{\lambda}})^{(i)},\mathcal{D}^{(i)}_{train},\mathcal{D}^{(i)}_{valid}),
}
\label{eq:pipeline_problem}
\end{equation}
where $\mathcal{D}_{train}$ and $\mathcal{D}_{valid}$ are training and validation datasets. Specifically, this equation minimises the k-fold cross validation error of loss function $\mathcal{L}$. The $k$ here is not to be confused with the $k$ variable used for predictor rankings elsewhere in this paper.




Equation (\ref{eq:pipeline_problem}) does not consider changes to the configuration space $\mathcal{T}$. If we reduce this configuration space by selecting promising pipelines to form the configuration subspace $\mathcal{T}^{*}\subset \mathcal{T}$, the problem of pipeline composition/optimisation can be reformulated as a constrained version of Eq. (\ref{eq:pipeline_problem}), as follows:  
\begin{equation}
\small{
(g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{*} = \mathrm{arg\,min}\frac{1}{k}\sum_{i=1}^{k} \mathcal{L}((g,\vec{\mathcal{A}}, \vec{\mathcal{\lambda}})^{(i)} \in \mathcal{T}',\mathcal{D}^{(i)}_{train},\mathcal{D}^{(i)}_{valid})
}
\label{eq:extended_pipeline_problem}
\end{equation}
subject to
\begin{equation}
\small{
%\mathcal{T}^{*} \subset \mathcal{T} \:\:\:\:\:  \textit{and} \:\:\:\:\:  h(\mathcal{T}^{*}) = \emptyset,
\mathcal{T}' = \mathcal{T}^{*}\setminus h(\mathcal{T}^{*}),
\label{eq:extended_pipeline_problem_constraints_1}
}
\end{equation}
where $h(\mathcal{T}^{*})$ is an optional function to find the set of all invalid pipelines. This set exclusion can be considered to represent the role of AVATAR \cite{ngga20}.




==> tables/tab_baseline.tex <==

\begin{landscape}

\begin{table*}[htb!]

\vspace{-0.35cm}

\caption {Baseline - the number of predictors have their rankings in top 8 well-performing predictors and the best ranking in top 8 well-performing predictors of all datasets.}
\label{tab:baseline}

\centering
%\tiny
\scriptsize


\begin{tabular}{|l|l|l|}
\hline
\textbf{Dataset}      & \textbf{\begin{tabular}[c]{@{}l@{}}The number of predictors have their rankings \\ in top 8 well-performing predictors\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}The best ranking in \\ top 8 well-performing predictors\end{tabular}} \\ \hline
\textbf{abalone}      & 3                                                                                                                                                    & 5                                                                                                                       \\ \hline
\textbf{adult}        & 5                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{amazon}       & 6                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{car}          & 5                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{cifar10small} & 4                                                                                                                                                    & 3                                                                                                                       \\ \hline
\textbf{convex}       & 4                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{dexter}       & 5                                                                                                                                                    & 4                                                                                                                       \\ \hline
\textbf{dorothea}     & 4                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{gcredit}      & 4                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{gisette}      & 5                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{kddcup}       & 1                                                                                                                                                    & 8                                                                                                                       \\ \hline
\textbf{krvskp}       & 6                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{madelon}      & 6                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{mnist}        & 4                                                                                                                                                    & 4                                                                                                                       \\ \hline
\textbf{secom}        & 1                                                                                                                                                    & 8                                                                                                                       \\ \hline
\textbf{semeion}      & 4                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{shuttle}      & 6                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{waveform}     & 5                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{winequality}  & 5                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{yeast}        & 7                                                                                                                                                    & 1                                                                                                                       \\ \hline
\end{tabular}


\end{table*}


\end{landscape}

==> tables/tab_compare_landmarking_and_no_landmarking.tex <==

\begin{landscape}

\begin{table*}[htb!]

\vspace{-0.35cm}
\captionsetup{font=scriptsize}
\caption {Compare mean, minimum and standard deviation without the AVATAR, with the AVATAR, and with the combination of the AVATAR and the relative landmarking.}
\label{tab:exp_error_compare}

\centering
%\tiny
\scriptsize


\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{l|}{\textbf{Mean Error Rate (\%)}}                   & \multicolumn{3}{l|}{\textbf{Minimum Error Rate (\%)}}                & \multicolumn{3}{l|}{\textbf{Standard Deviation of Error Rate}}       \\ \cline{2-10} 
                                  & \textbf{No Avatar} & \textbf{Avatar} & \textbf{Avatar + Landmarking} & \textbf{No Avatar} & \textbf{Avatar} & \textbf{Avatar + Landmarking} & \textbf{No Avatar} & \textbf{Avatar} & \textbf{Avatar + Landmarking} \\ \hline
\textbf{abalone}                  & 73.5               & 73.9            & \textbf{73.4}                 & 73.2               & \textbf{72.9}   & 73.1                          & 0.2                & 0.9             & 0.4                           \\ \hline
\textbf{adult}                    & \textbf{14.4}      & 14.6            & \textbf{14.4}                 & \textbf{13.4}      & \textbf{13.4}   & \textbf{13.4}                 & 0.7                & 0.6             & 0.6                           \\ \hline
\textbf{amazon}                   & 58.6               & 46.0            & \textbf{38.5}                 & 52.2               & \textbf{38.5}   & \textbf{38.5}                 & 6.4                & 10.7            & 0.0                           \\ \hline
\textbf{car}                      & 2.7                & 0.6             & \textbf{0.3}                  & 1.1                & \textbf{0.3}    & \textbf{0.3}                  & 0.9                & 0.3             & 0.0                           \\ \hline
\textbf{cifar10small}             & 75.4               & 71.9            & \textbf{65.5}                 & 66.6               & 64.9            & \textbf{60.6}                 & 8.9                & 8.8             & 4.9                           \\ \hline
\textbf{convex}                   & 39.0               & 33.5            & \textbf{31.1}                 & 35.9               & 25.7            & \textbf{21.5}                 & 2.4                & 5.7             & 6.4                           \\ \hline
\textbf{dexter}                   & 8.8                & \textbf{8.1}    & 8.9                           & 8.8                & \textbf{6.9}    & 8.6                           & 0.0                & 0.8             & 0.2                           \\ \hline
\textbf{dorothea}                 & 9.3                & 8.0             & \textbf{6.7}                  & 9.3                & \textbf{6.7}    & \textbf{6.7}                  & 0.0                & 1.3             & 0.0                           \\ \hline
\textbf{gcredit}                  & 22.8               & \textbf{22.3}   & 22.4                          & 22.4               & \textbf{21.7}   & \textbf{21.7}                 & 0.3                & 0.4             & 0.4                           \\ \hline
\textbf{gisette}                  & 2.9                & \textbf{2.6}    & 6.6                           & 2.4                & \textbf{2.4}    & 6.6                           & 0.5                & 0.2             & 0.0                           \\ \hline
\textbf{kddcup}                   & \textbf{1.8}       & \textbf{1.8}    & \textbf{1.8}                  & 1.8                & \textbf{1.8}    & \textbf{1.8}                  & 0.0                & 0.0             & 0.0                           \\ \hline
\textbf{krvskp}                   & 0.7                & \textbf{0.4}    & \textbf{0.4}                  & 0.5                & \textbf{0.4}    & \textbf{0.4}                  & 0.1                & 0.0             & 0.0                           \\ \hline
\textbf{madelon}                  & 26.0               & 22.9            & \textbf{22.7}                 & 22.8               & 22.8            & \textbf{22.6}                 & 3.3                & 0.2             & 0.1                           \\ \hline
\textbf{mnist}                    & -                  & \textbf{16.4}   & -                             & -                  & \textbf{16.4}   & -                             & -                  & 0.0             & -                             \\ \hline
\textbf{secom}                    & \textbf{6.1}       & \textbf{6.1}    & \textbf{6.1}                  & \textbf{6.1}       & \textbf{6.1}    & \textbf{6.1}                  & 0.0                & 0.0             & 0.0                           \\ \hline
\textbf{semeion}                  & 8.4                & 4.9             & \textbf{4.6}                  & 5.6                & 4.7             & \textbf{4.3}                  & 2.0                & 0.4             & 0.3                           \\ \hline
\textbf{shuttle}                  & 0.0                & 0.1             & \textbf{0.0}                  & \textbf{0.0}       & \textbf{0.0}    & \textbf{0.0}                  & 0.0                & 0.1             & 0.0                           \\ \hline
\textbf{waveform}                 & 12.7               & \textbf{12.5}   & \textbf{12.5}                 & 12.7               & \textbf{12.5}   & \textbf{12.5}                 & 0.1                & 0.1             & 0.1                           \\ \hline
\textbf{winequality}              & 37.8               & \textbf{33.4}   & 33.9                          & 33.4               & \textbf{33.1}   & 32.4                          & 5.7                & 0.4             & 1.3                           \\ \hline
\textbf{yeast}                    & 39.2               & 38.0            & \textbf{37.9}                 & 38.5               & 37.0            & \textbf{36.9}                 & 0.5                & 0.6             & 0.5                           \\ \hline
\end{tabular}


\end{table*}


\end{landscape}

==> tables/tab_dataset.tex <==
\begin{table}[htb!]
\centering
%\vspace{-0.65cm}
\caption {Dataset characteristics: the number of numeric attributes, nominal attributes, the number of distinct classes, instances in training and testing sets.}
\label{tab:datasets}
%\scriptsize
\fontsize{7.2}{8.5}\selectfont
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Dataset}  & \textbf{Numeric} & \textbf{Nominal} & \textbf{Distinct classes} & \textbf{Train} & \textbf{Test} \\ \hline
abalone           & 7                & 1                & 28                              & 2,924          & 1,253         \\ \hline
adult             & 6                & 8                & 2                               & 32,561         & 16,281        \\ \hline
amazon            & 10,000           & 0                & 50                              & 1,050          & 450           \\ \hline
car               & 0                & 6                & 4                               & 1,210          & 518           \\ \hline
cifar10small      & 3,072            & 0                & 10                              & 10,000         & 10,000        \\ \hline
convex            & 784              & 0                & 2                               & 8,000          & 50,000        \\ \hline
dexter            & 20,000           & 0                & 2                               & 420            & 180           \\ \hline
dorothea          & 100,000          & 0                & 2                               & 805            & 345           \\ \hline
gcredit           & 7                & 13               & 2                               & 700            & 300           \\ \hline
gisette           & 5,000            & 0                & 2                               & 4,900          & 2,100         \\ \hline
kddcup & 192              & 38               & 2                               & 35,000         & 15,000        \\ \hline
krvskp            & 0                & 36               & 2                               & 2,238          & 958           \\ \hline
madelon           & 500              & 0                & 2                               & 1,820          & 780           \\ \hline
mnist             & 784              & 0                & 10                              & 12,000         & 50,000        \\ \hline
secom             & 590              & 0                & 2                               & 1,097          & 470           \\ \hline
semeion           & 256              & 0                & 10                              & 1,116          & 477           \\ \hline
shuttle           & 9                & 0                & 7                               & 43,500         & 14,500        \\ \hline
waveform          & 40               & 0                & 3                               & 3,500          & 1,500         \\ \hline
winequality       & 11               & 0                & 11                              & 3,429          & 1,469         \\ \hline
yeast             & 8                & 0                & 10                              & 1,039          & 445           \\ \hline
\end{tabular}

\end{table}

==> tables/tab_error_all_methods.tex <==


\begin{table*}[htb!]

\vspace{-0.35cm}

\caption {Mean error rate (\%) of the pipelines found by SMAC using different configuration spaces.   }
\label{tab:error_rate_all_methods}

\centering
%\tiny
%\scriptsize
%\fontsize{5.8}{8}\selectfont
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Dataset}      & \textbf{baseline} & \textbf{r30}   & \textbf{avatar} & \textbf{L-k1}  & \textbf{L-k4}  & \textbf{L-k8} & \textbf{L-k10} & \textbf{L-k19} & \textbf{O-k1}  & \textbf{O-k4}  & \textbf{O-k8}  & \textbf{O-k10} & \textbf{O-k19} \\ \hline
\textbf{abalone}      & 73.46             & 73.81          & 73.85           & \textbf{72.74} & 72.95          & 73.40         & 72.98          & 73.27          & 73.77          & 73.42          & 73.31          & 73.28          & 72.93          \\ \hline
\textbf{adult}        & 13.41             & 13.22          & 13.41           & \textbf{12.87} & 14.89          & 14.86         & 13.99          & 14.16          & -              & 13.72          & 13.92          & 13.77          & 13.62          \\ \hline
\textbf{amazon}       & 58.57             & \textbf{29.33} & 46.03           & 74.23          & 31.79          & 38.48         & 38.48          & 44.06          & -              & 38.48          & 38.48          & 38.48          & 41.90          \\ \hline
\textbf{car}          & 2.73              & 0.35           & 0.58            & \textbf{0.33}  & 0.35           & \textbf{0.33} & \textbf{0.33}  & 0.38           & 2.60           & 0.35           & 0.36           & \textbf{0.33}  & 0.55           \\ \hline
\textbf{cifar10small} & 75.40             & 66.66          & 71.90           & 83.42          & 70.98          & 68.15         & 70.42          & -              & -              & 64.78          & \textbf{57.70} & 70.72          & 62.35          \\ \hline
\textbf{convex}       & 38.99             & 46.72          & 30.64           & -              & 38.79          & 34.25         & 25.65          & 30.13          & -              & 26.83          & \textbf{25.51} & 28.76          & 31.31          \\ \hline
\textbf{dexter}       & 8.81              & 8.21           & 8.10            & \textbf{5.33}  & 7.19           & 8.05          & 7.90           & 8.95           & 6.29           & 5.67           & 7.80           & 8.39           & 8.93           \\ \hline
\textbf{dorothea}     & 9.30              & 7.21           & 6.71            & -              & -              & -             & 6.71           & 6.71           & 6.71           & 6.34           & 6.34           & \textbf{5.47}  & 7.21           \\ \hline
\textbf{gcredit}      & 22.83             & 23.26          & 22.26           & 23.49          & 23.00          & 23.00         & 22.57          & 22.14          & 23.00          & \textbf{21.23} & 21.49          & 21.91          & 21.80          \\ \hline
\textbf{gisette}      & 2.93              & \textbf{1.80}  & 2.57            & 3.22           & -              & 6.55          & 6.41           & 4.18           & 2.06           & 2.48           & 2.43           & 2.36           & 2.93           \\ \hline
\textbf{kddcup}       & \textbf{1.80}     & -              & \textbf{1.80}   & -              & -              & -             & -              & -              & \textbf{1.80}  & \textbf{1.80}  & \textbf{1.80}  & -              & \textbf{1.80}  \\ \hline
\textbf{krvskp}       & 0.67              & \textbf{0.38}  & 0.44            & 0.78           & 0.74           & 0.40          & 0.40           & 0.43           & 0.55           & 0.41           & 0.42           & 0.44           & 0.46           \\ \hline
\textbf{madelon}      & 26.04             & 39.41          & 22.86           & 33.84          & \textbf{22.66} & 22.68         & 22.68          & 22.88          & \textbf{22.66} & 22.72          & 23.04          & 22.91          & 23.41          \\ \hline
\textbf{mnist}        & -                 & 9.01           & 16.38           & -              & -              & -             & 2.71           & 9.12           & 3.96           & -              & \textbf{2.68}  & 7.42           & 7.54           \\ \hline
\textbf{secom}        & 6.11              & \textbf{6.06}  & 6.11            & -              & 6.11           & 6.11          & 6.11           & 6.11           & 6.11           & 6.11           & 6.11           & 6.11           & 6.11           \\ \hline
\textbf{semeion}      & 8.37              & 5.47           & 4.95            & 4.46           & \textbf{4.45}  & 4.53          & 4.59           & 5.36           & 8.65           & 4.77           & 5.41           & 5.52           & 6.93           \\ \hline
\textbf{shuttle}      & 0.03              & \textbf{0.02}  & 0.09            & 0.25           & 0.04           & 0.03          & 0.03           & 0.04           & \textbf{0.02}  & \textbf{0.02}  & \textbf{0.02}  & \textbf{0.02}  & 0.03           \\ \hline
\textbf{waveform}     & 12.71             & 12.90          & 12.53           & \textbf{12.44} & 12.55          & 12.46         & 12.47          & 12.58          & 12.57          & 12.50          & 12.57          & 12.54          & 12.49          \\ \hline
\textbf{winequality}  & 37.84             & 34.57          & 33.52           & 39.01          & 33.21          & 33.56         & 33.45          & 33.92          & \textbf{32.72} & 32.91          & 32.89          & 33.29          & 35.19          \\ \hline
\textbf{yeast}        & 39.15             & 39.94          & 38.02           & 41.20          & 38.52          & 37.80         & 37.94          & 37.80          & \textbf{36.65} & 36.90          & 37.63          & 37.42          & 37.55          \\ \hline
\end{tabular}


\end{table*}



==> tables/tab_error_all_methods_ranking.tex <==


\begin{table}[htb!]

\vspace{-0.35cm}

\caption {Ranking of mean error rate (\%) of the pipelines found by SMAC using different configuration spaces.   }
\label{tab:error_rate_all_methods_ranking}

\centering
%\tiny
\scriptsize

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Dataset}      & \textbf{best known} & \textbf{no avatar} & \textbf{avatar} & \textbf{L-k1} & \textbf{L-k4} & \textbf{L-k8} & \textbf{L-k10} & \textbf{L-k19} & \textbf{O-k1} & \textbf{O-k4} & \textbf{O-k8} & \textbf{O-k10} & \textbf{O-k19} \\ \hline
\textbf{abalone}      & 12.0                & 10.0               & 13.0            & \textbf{1.0}  & 3.0           & 8.0           & 4.0            & 5.0            & 11.0          & 9.0           & 7.0           & 6.0            & 2.0            \\ \hline
\textbf{adult}        & 2.0                 & 3.5                & 3.5             & \textbf{1.0}  & 12.0          & 11.0          & 9.0            & 10.0           & 13.0          & 6.0           & 8.0           & 7.0            & 5.0            \\ \hline
\textbf{amazon}       & \textbf{1.0}        & 11.0               & 10.0            & 12.0          & 2.0           & 5.0           & 5.0            & 9.0            & 13.0          & 5.0           & 5.0           & 5.0            & 8.0            \\ \hline
\textbf{car}          & 6.0                 & 13.0               & 11.0            & \textbf{2.5}  & 6.0           & \textbf{2.5}  & \textbf{2.5}   & 9.0            & 12.0          & 6.0           & 8.0           & \textbf{2.5}   & 10.0           \\ \hline
\textbf{cifar10small} & 4.0                 & 10.0               & 9.0             & 11.0          & 8.0           & 5.0           & 6.0            & 12.5           & 12.5          & 3.0           & \textbf{1.0}  & 7.0            & 2.0            \\ \hline
\textbf{convex}       & 11.0                & 10.0               & 6.0             & 12.5          & 9.0           & 8.0           & 2.0            & 5.0            & 12.5          & 3.0           & \textbf{1.0}  & 4.0            & 7.0            \\ \hline
\textbf{dexter}       & 9.0                 & 11.0               & 8.0             & \textbf{1.0}  & 4.0           & 7.0           & 6.0            & 13.0           & 3.0           & 2.0           & 5.0           & 10.0           & 12.0           \\ \hline
\textbf{dorothea}     & 8.5                 & 10.0               & 5.5             & 12.0          & 12.0          & 12.0          & 5.5            & 5.5            & 5.5           & 2.5           & 2.5           & \textbf{1.0}   & 8.5            \\ \hline
\textbf{gcredit}      & 12.0                & 8.0                & 6.0             & 13.0          & 10.0          & 10.0          & 7.0            & 5.0            & 10.0          & \textbf{1.0}  & 2.0           & 4.0            & 3.0            \\ \hline
\textbf{gisette}      & \textbf{1.0}        & 7.0                & 6.0             & 9.0           & 13.0          & 12.0          & 11.0           & 10.0           & 2.0           & 5.0           & 4.0           & 3.0            & 8.0            \\ \hline
\textbf{kddcup}       & 10.0                & \textbf{3.5}       & \textbf{3.5}    & 10.0          & 10.0          & 10.0          & 10.0           & 10.0           & \textbf{3.5}  & \textbf{3.5}  & \textbf{3.5}  & 10.0           & \textbf{3.5}   \\ \hline
\textbf{krvskp}       & \textbf{1.0}        & 11.0               & 7.5             & 13.0          & 12.0          & 2.5           & 2.5            & 6.0            & 10.0          & 4.0           & 5.0           & 7.5            & 9.0            \\ \hline
\textbf{madelon}      & 13.0                & 11.0               & 6.0             & 12.0          & \textbf{1.0}  & 3.5           & 3.5            & 7.0            & 2.0           & 5.0           & 9.0           & 8.0            & 10.0           \\ \hline
\textbf{mnist}        & 6.0                 & 11.0               & 8.0             & 11.0          & 11.0          & 11.0          & 2.0            & 7.0            & 3.0           & 11.0          & \textbf{1.0}  & 4.0            & 5.0            \\ \hline
\textbf{secom}        & \textbf{1.0}        & 7.0                & 7.0             & 13.0          & 7.0           & 7.0           & 7.0            & 7.0            & 7.0           & 7.0           & 7.0           & 7.0            & 7.0            \\ \hline
\textbf{semeion}      & 9.0                 & 12.0               & 6.0             & 2.0           & \textbf{1.0}  & 3.0           & 4.0            & 7.0            & 13.0          & 5.0           & 8.0           & 10.0           & 11.0           \\ \hline
\textbf{shuttle}      & 5.0                 & 9.0                & 12.0            & 13.0          & 11.0          & 8.0           & 6.0            & 10.0           & \textbf{1.0}  & 3.0           & 2.0           & 4.0            & 7.0            \\ \hline
\textbf{waveform}     & 13.0                & 12.0               & 6.0             & \textbf{1.0}  & 8.0           & 2.0           & 3.0            & 11.0           & 9.0           & 5.0           & 10.0          & 7.0            & 4.0            \\ \hline
\textbf{winequality}  & 10.0                & 12.0               & 7.0             & 13.0          & 4.0           & 8.0           & 6.0            & 9.0            & \textbf{1.0}  & 3.0           & 2.0           & 5.0            & 11.0           \\ \hline
\textbf{yeast}        & 12.0                & 11.0               & 9.0             & 13.0          & 10.0          & 6.0           & 8.0            & 7.0            & \textbf{1.0}  & 2.0           & 5.0           & 3.0            & 4.0            \\ \hline
\end{tabular}



\end{table}



==> tables/tab_historical_runs_predictors_and_mean_error.tex <==

\begin{landscape}

\begin{table*}[htb!]

\vspace{-0.35cm}

\caption {Mean error rate (\%) of ML pipelines containing predictors that is extracted from prior evaluations of 20 datasets. Symbol '-' presents that SMAC haven't evaluated the pipelines containing the predictors.}
\label{tab:historical_runs_predictors_mean_erros}

\centering
\tiny
%\scriptsize
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{dataset}                                                                   & \textbf{abalone} & \textbf{adult} & \textbf{amazon} & \textbf{car} & \textbf{\begin{tabular}[c]{@{}l@{}}cifar\\ 10small\end{tabular}} & \textbf{convex} & \textbf{dexter} & \textbf{dorothea} & \textbf{gcredit} & \textbf{gisette} & \textbf{kddcup} & \textbf{krvskp} & \textbf{madelon} & \textbf{mnist} & \textbf{secom} & \textbf{semeion} & \textbf{shuttle} & \textbf{waveform} & \textbf{\begin{tabular}[c]{@{}l@{}}wine\\ quality\end{tabular}} & \textbf{yeast} \\ \hline
\textbf{JRip}                                                                      & 80.6             & 22.0           & 66.5            & 17.5         & 75.9                                                             & 39.4            & 17.1            & 7.0               & 27.4             & 6.3              & 1.8             & 1.9             & 26.7             & 15.5           & 7.5            & 29.5             & 1.2              & 22.2              & 47.4                                                            & 44.9           \\ \hline
\textbf{REPTree}                                                                   & 75.9             & 15.5           & 83.6            & 16.9         & 75.0                                                             & 45.5            & 21.4            & 14.8              & 28.8             & 7.7              & -               & 3.6             & 26.9             & 29.2           & 6.4            & 36.4             & 0.6              & 25.1              & 48.2                                                            & 45.8           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Decision\\ Table\end{tabular}}                  & 74.0             & 15.0           & 78.1            & 19.4         & 74.7                                                             & 47.2            & 24.4            & -                 & 29.9             & 9.8              & 1.8             & 5.8             & 31.7             & 90.5           & 6.6            & 56.3             & 0.3              & 38.5              & 48.6                                                            & 46.7           \\ \hline
\textbf{LMT}                                                                       & 75.0             & 13.9           & 36.2            & 7.1          & -                                                                & -               & 28.6            & -                 & 26.1             & -                & -               & 1.3             & 34.9             & 90.3           & 6.7            & 17.1             & 0.2              & 15.1              & 48.4                                                            & 45.3           \\ \hline
\textbf{J48}                                                                       & 76.3             & 14.4           & 63.8            & 11.7         & 72.7                                                             & 39.6            & 17.3            & 7.5               & 27.8             & 7.6              & 1.9             & 1.6             & 38.0             & 18.2           & 6.6            & 31.5             & 0.9              & 24.9              & 46.8                                                            & 45.3           \\ \hline
\textbf{PART}                                                                      & 75.8             & 14.2           & 65.9            & 10.9         & 72.9                                                             & 38.5            & 20.5            & 8.7               & 27.8             & 7.8              & 1.8             & 3.8             & 38.7             & 16.4           & 7.3            & 30.9             & 0.7              & 23.2              & 46.3                                                            & 45.0           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Decision\\ Stump\end{tabular}}                  & 81.1             & 24.3           & 98.2            & 32.4         & 84.0                                                             & 47.9            & 32.0            & 6.8               & 30.2             & 16.0             & 1.8             & 34.1            & 39.6             & 81.4           & 6.0            & 82.5             & 14.9             & 43.3              & 55.9                                                            & 60.4           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Random\\ Forest\end{tabular}}                   & 76.1             & 15.9           & 82.6            & 11.2         & 67.7                                                             & 30.7            & 24.5            & 9.5               & 25.2             & 7.0              & 23.6            & 4.4             & 41.7             & 25.3           & 6.1            & 15.9             & 0.0              & 19.7              & 37.6                                                            & 41.3           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}NaiveBayes\\ Multinomial\end{tabular}}          & -                & -              & 38.5            & -            & 71.2                                                             & 49.3            & 9.2             & 8.6               & -                & 7.8              & -               & -               & 42.2             & 17.4           & -              & 15.6             & 21.3             & 62.9              & 60.2                                                            & 68.2           \\ \hline
\textbf{NaiveBayes}                                                                & 75.7             & 16.1           & 52.8            & 17.0         & 71.2                                                             & 47.7            & 10.9            & 7.4               & 23.8             & 12.1             & 2.9             & 15.3            & 42.4             & 44.5           & 45.7           & 15.1             & 4.4              & 20.2              & 53.4                                                            & 42.1           \\ \hline
\textbf{OneR}                                                                      & 76.1             & 24.7           & 95.1            & 30.9         & 82.6                                                             & 47.9            & 35.9            & 7.5               & 34.2             & 15.2             & 2.9             & 32.1            & 42.8             & 74.5           & 7.2            & 82.8             & 5.2              & 46.4              & 54.2                                                            & 61.4           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Voted\\ Perceptron\end{tabular}}                & -                & 21.1           & -               & -            & -                                                                & 37.5            & 10.2            & 7.8               & 42.2             & 2.6              & -               & 3.9             & 43.7             & -              & 6.2            & -                & -                & -                 & -                                                               & -              \\ \hline
\textbf{RBFKernel}                                                                 & 75.3             & 20.5           & 95.2            & 14.7         & 54.2                                                             & 28.2            & 50.4            & -                 & 27.5             & 50.7             & -               & 9.3             & 43.9             & 7.4            & 7.6            & 15.9             & 6.6              & 22.1              & 48.6                                                            & 47.9           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Simple\\ Logistic\end{tabular}}                 & 75.6             & 15.6           & 58.7            & 15.7         & 90.5                                                             & 46.4            & 12.1            & 7.6               & 26.1             & 3.1              & -               & 11.4            & 44.1             & 18.8           & 7.0            & 17.0             & 10.1             & 13.8              & 51.4                                                            & 47.2           \\ \hline
\textbf{SMO}                                                                       & 75.7             & 31.6           & 79.6            & 9.4          & 62.2                                                             & 31.9            & 49.6            & 14.8              & 26.9             & 19.3             & -               & 8.9             & 44.9             & 7.4            & 6.7            & 15.3             & 5.8              & 23.6              & 52.9                                                            & 46.7           \\ \hline
\textbf{Logistic}                                                                  & 73.9             & 15.0           & 67.9            & 9.5          & -                                                                & 47.9            & -               & -                 & 24.7             & 7.3              & -               & 4.1             & 45.1             & 25.2           & 14.7           & 10.9             & 3.1              & 13.1          & 47.1                                                            & 41.7           \\ \hline
\textbf{SGD}                                                                       & -                & 17.5           & -               & -            & -                                                                & 45.8            & 7.9             & -                 & 26.9             & 3.4              & -               & 7.4             & 45.2             & -              & 9.9            & -                & -                & -                 & -                                                               & -              \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}AdaBoost\\ M1\end{tabular}}                     & 87.9             & 22.0           & -               & 36.2         & -                                                                & 44.8            & 61.9            & -                 & 31.7             & -                & 1.8             & 29.6            & 47.0             & -              & 13.8           & 68.6             & 29.6             & 36.2              & 68.6                                                            & 69.5           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Random\\ SubSpace\end{tabular}}                 & 80.1             & 24.5           & -               & 40.3         & 81.7                                                             & 47.3            & -               & -                 & 34.0             & -                & -               & 34.3            & 47.2             & 32.3           & 6.2            & 42.1             & 42.4             & 28.1              & 69.5                                                            & 63.0           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Random\\ Tree\end{tabular}}                     & 77.6             & 16.2           & 94.8            & 21.4         & 78.4                                                             & 40.9            & 37.2            & 11.7              & 30.7             & 19.1             & 3.0             & 14.2            & 47.9             & 31.8           & 7.2            & 50.8             & 0.4              & 30.2              & 49.5                                                            & 48.1           \\ \hline
\textbf{IBk}                                                                       & 81.6             & 26.2           & 91.4            & 29.1         & 88.6                                                             & 49.6            & 53.6            & -                 & 31.6             & 21.2             & 1.8             & 34.7            & 48.7             & 40.9           & 7.0            & 52.3             & 15.2             & 39.7              & 58.7                                                            & 59.0           \\ \hline
\textbf{Bagging}                                                                   & 74.8             & 24.6           & -               & 40.7         & 90.5                                                             & -               & -               & -                 & 31.5             & -                & -               & 33.5            & 49.0             & -              & 12.8           & 84.4             & 16.9             & 28.1              & 59.7                                                            & 55.0           \\ \hline
\textbf{Vote}                                                                      & 99.7             & 24.6           & -               & 40.5         & -                                                                & -               & -               & -                 & 33.1             & -                & -               & 36.2            & 49.5             & -              & -              & -                & -                & 45.1              & 48.1                                                            & 91.3           \\ \hline
\textbf{LogitBoost}                                                                & 88.5             & -              & -               & 33.5         & -                                                                & -               & -               & -                 & 32.7             & -                & -               & 41.9            & 49.5             & -              & 5.5            & 36.0             & -                & 32.4              & 71.4                                                            & 66.8           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Multilayer\\ Perceptron\end{tabular}}           & 76.6             & 15.8           & -               & 19.1    & -                                                                & 48.3            & -               & -                 & 25.5             & -                & 1.8             & 20.7            & 49.8             & 90.7           & 6.1            & 23.5             & 20.3             & 16.6              & 57.1                                                            & 56.8           \\ \hline
\textbf{KStar}                                                                     & 75.0             & 20.7           & 98.1            & 27.7         & 92.7                                                             & 47.2            & 49.6            & 25.7              & 29.8             & 49.4             & 1.8             & 6.5             & 49.9             & 11.3           & 6.1            & 35.4             & 4.6              & 29.5              & 39.1                                                            & 54.5           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Classification\\ ViaRegression\end{tabular}}    & 94.0             & -              & -               & 36.3         & -                                                                & -               & -               & -                 & 40.5             & -                & -               & 32.2            & 51.1             & -              & 6.1            & 85.7             & 14.5             & 53.9              & 64.5                                                            & 69.8           \\ \hline
\textbf{ZeroR}                                                                     & 83.8             & 24.2           & 99.4            & 34.4         & 90.3                                                             & 51.0            & 57.3            & 9.7               & 30.2             & 50.0             & 1.8             & 47.5            & 51.5             & 89.2           & 6.1            & 90.5             & 25.7             & 66.1              & 56.9                                                            & 71.1           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Attribute\\ Selected\\ Classifier\end{tabular}} & 88.4             & 23.6           & 97.1            & 40.8         & 90.5                                                             & -               & -               & -                 & 42.6             & 13.7             & -               & 29.4            & 51.8             & 90.8           & -              & 88.4             & 47.7             & 55.4              & 69.3                                                            & 78.7           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}MultiClass\\ Classifier\end{tabular}}           & 90.4             & 23.7-735       & -               & 44.8         & -                                                                & 47.5            & -               & -                 & 35.5             & -                & 1.7             & 34.1            & -                & -              & 6.1            & 53.1             & 11.1             & 50.2              & 59.4                                                            & 85.1           \\ \hline
\end{tabular}

\end{table*}


\end{landscape}

==> tables/tab_histotical_runs_predictors_and_ranking_mean_error.tex <==

\begin{landscape}

\begin{table*}[htb!]

\vspace{-0.35cm}
\captionsetup{font=scriptsize}
\caption {Ranking of predictors based on mean error rate of their pipelines that is extracted from historical runs of 20 datasets within 2 hours optimisation time.}
\label{tab:historical_runs_predictors_mean_erros_ranking}

\centering
\tiny
%\scriptsize


\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{dataset}                                                                   & \textbf{abalone} & \textbf{adult} & \textbf{amazon} & \textbf{car} & \textbf{\begin{tabular}[c]{@{}l@{}}cifar\\ 10small\end{tabular}} & \textbf{convex} & \textbf{dexter} & \textbf{dorothea} & \textbf{gcredit} & \textbf{gisette} & \textbf{kddcup} & \textbf{krvskp} & \textbf{madelon} & \textbf{mnist} & \textbf{secom} & \textbf{semeion} & \textbf{shuttle} & \textbf{waveform} & \textbf{\begin{tabular}[c]{@{}l@{}}wine\\ quality\end{tabular}} & \textbf{yeast} \\ \hline
\textbf{NaiveBayes}                                                                & 8                & 10             & 3               & 10           & 5                                                                & 17              & 4               & 3                 & 1                & 12               & 13              & 16              & 10               & 15             & 27             & 2                & 10               & 6                 & 15                                                              & 3              \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}NaiveBayes\\ Multinomial\end{tabular}}          & 28               & 28             & 2               & 28           & 4                                                                & 22              & 2               & 8                 & 30               & 10               & 16              & 30              & 9                & 6              & 28             & 4                & 22               & 27                & 23                                                              & 22             \\ \hline
\textbf{Logistic}                                                                  & 1                & 5              & 8               & 3            & 21                                                               & 19              & 22              & 16                & 2                & 6                & 16              & 7               & 16               & 9              & 26             & 1                & 9                & 1                 & 5                                                               & 2              \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Multilayer\\ Perceptron\end{tabular}}           & 15               & 8              & 21              & 12           & 21                                                               & 21              & 22              & 16                & 4                & 22               & 2               & 17              & 25               & 21             & 7              & 9                & 21               & 4                 & 19                                                              & 16             \\ \hline
\textbf{SGD}                                                                       & 28               & 12             & 21              & 28           & 21                                                               & 11              & 1               & 16                & 8                & 3                & 16              & 11              & 17               & 23             & 23             & 28               & 27               & 29                & 29                                                              & 29             \\ \hline
\textbf{SimpleLogistic}                                                            & 7                & 7              & 4               & 8            & 17                                                               & 12              & 5               & 6                 & 5                & 2                & 16              & 14              & 14               & 8              & 16             & 7                & 15               & 2                 & 13                                                              & 11             \\ \hline
\textbf{SMO}                                                                       & 9                & 27             & 10              & 2            & 2                                                                & 3               & 17              & 14                & 7                & 17               & 16              & 12              & 15               & 1              & 14             & 3                & 13               & 10                & 14                                                              & 9              \\ \hline
\textbf{RBFKernel}                                                                 & 6                & 13             & 16              & 7            & 1                                                                & 1               & 18              & 16                & 10               & 21               & 16              & 13              & 13               & 1              & 22             & 5                & 14               & 7                 & 11                                                              & 12             \\ \hline
\textbf{VotedPerceptron}                                                           & 28               & 15             & 21              & 28           & 21                                                               & 4               & 3               & 7                 & 28               & 1                & 16              & 6               & 12               & 23             & 10             & 28               & 27               & 29                & 29                                                              & 29             \\ \hline
\textbf{IBk}                                                                       & 20               & 26             & 13              & 16           & 15                                                               & 23              & 19              & 16                & 20               & 18               & 4               & 26              & 21               & 14             & 17             & 18               & 19               & 20                & 20                                                              & 17             \\ \hline
\textbf{KStar}                                                                     & 4                & 14             & 18              & 15           & 20                                                               & 14              & 16              & 15                & 14               & 19               & 7               & 10              & 26               & 3              & 6              & 13               & 11               & 15                & 2                                                               & 14             \\ \hline
\textbf{AdaBoostM1}                                                                & 22               & 16             & 21              & 21           & 21                                                               & 9               & 21              & 16                & 21               & 22               & 8               & 19              & 18               & 23             & 25             & 21               & 24               & 18                & 25                                                              & 23             \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Attribute\\ Selected\\ Classifier\end{tabular}} & 23               & 18             & 17              & 26           & 17                                                               & 25              & 22              & 16                & 29               & 13               & 16              & 18              & 29               & 22             & 28             & 26               & 26               & 26                & 26                                                              & 26             \\ \hline
\textbf{Bagging}                                                                   & 3                & 23             & 21              & 25           & 17                                                               & 25              & 22              & 16                & 19               & 22               & 16              & 22              & 22               & 23             & 24             & 24               & 20               & 13                & 22                                                              & 15             \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Classification\\ ViaRegression\end{tabular}}    & 26               & 28             & 21              & 22           & 21                                                               & 25              & 22              & 16                & 27               & 22               & 16              & 21              & 27               & 23             & 4              & 25               & 17               & 25                & 24                                                              & 24             \\ \hline
\textbf{LogitBoost}                                                                & 24               & 28             & 21              & 19           & 21                                                               & 25              & 22              & 16                & 22               & 22               & 16              & 28              & 23               & 23             & 1              & 14               & 27               & 17                & 28                                                              & 21             \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}MultiClass\\ Classifier\end{tabular}}           & 25               & 19             & 21              & 27           & 21                                                               & 16              & 22              & 16                & 26               & 22               & 1               & 24              & 30               & 23             & 4              & 19               & 16               & 24                & 21                                                              & 27             \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Random\\ SubSpace\end{tabular}}                 & 17               & 22             & 21              & 23           & 12                                                               & 15              & 22              & 16                & 24               & 22               & 16              & 25              & 19               & 13             & 9              & 16               & 25               & 14                & 27                                                              & 20             \\ \hline
\textbf{Vote}                                                                      & 27               & 23             & 21              & 24           & 21                                                               & 25              & 22              & 16                & 23               & 22               & 16              & 27              & 23               & 23             & 28             & 28               & 27               & 22                & 7                                                               & 28             \\ \hline
\textbf{DecisionTable}                                                             & 2                & 4              & 9               & 13           & 8                                                                & 13              & 10              & 16                & 15               & 11               & 6               & 9               & 3                & 20             & 12             & 20               & 3                & 19                & 10                                                              & 10             \\ \hline
\textbf{JRip}                                                                      & 18               & 17             & 7               & 11           & 10                                                               & 6               & 6               & 2                 & 9                & 4                & 8               & 3               & 1                & 4              & 21             & 10               & 8                & 8                 & 6                                                               & 4              \\ \hline
\textbf{OneR}                                                                      & 12               & 25             & 15              & 17           & 13                                                               & 18              & 14              & 5                 & 25               & 14               & 12              & 20              & 11               & 16             & 19             & 23               & 12               & 23                & 16                                                              & 19             \\ \hline
\textbf{PART}                                                                      & 10               & 2              & 6               & 4            & 7                                                                & 5               & 8               & 9                 & 11               & 9                & 10              & 5               & 6                & 5              & 20             & 11               & 6                & 9                 & 3                                                               & 5              \\ \hline
\textbf{ZeroR}                                                                     & 21               & 20             & 20              & 20           & 16                                                               & 24              & 20              & 11                & 16               & 20               & 4               & 29              & 28               & 18             & 3              & 27               & 23               & 28                & 18                                                              & 25             \\ \hline
\textbf{DecisionStump}                                                             & 19               & 21             & 19              & 18           & 14                                                               & 20              & 13              & 1                 & 17               & 15               & 3               & 23              & 7                & 17             & 2              & 22               & 18               & 21                & 17                                                              & 18             \\ \hline
\textbf{J48}                                                                       & 14               & 3              & 5               & 6            & 6                                                                & 7               & 7               & 4                 & 12               & 7                & 11              & 2               & 5                & 7              & 13             & 12               & 7                & 11                & 4                                                               & 6              \\ \hline
\textbf{LMT}                                                                       & 5                & 1              & 1               & 1            & 21                                                               & 25              & 12              & 16                & 6                & 22               & 16              & 1               & 4                & 19             & 15             & 8                & 2                & 3                 & 9                                                               & 7              \\ \hline
\textbf{RandomForest}                                                              & 13               & 9              & 11              & 5            & 3                                                                & 2               & 11              & 10                & 3                & 5                & 15              & 8               & 8                & 10             & 8              & 6                & 1                & 5                 & 1                                                               & 1              \\ \hline
\textbf{RandomTree}                                                                & 16               & 11             & 14              & 14           & 11                                                               & 8               & 15              & 12                & 18               & 16               & 14              & 15              & 20               & 12             & 18             & 17               & 4                & 16                & 12                                                              & 13             \\ \hline
\textbf{REPTree}                                                                   & 11               & 6              & 12              & 9            & 9                                                                & 10              & 9               & 13                & 13               & 8                & 16              & 4               & 2                & 11             & 11             & 15               & 5                & 12                & 8                                                               & 8              \\ \hline
\end{tabular}


\end{table*}


\end{landscape}

==> tables/tab_landmarking_results_extractedhistory.tex <==



\begin{table}[htb!]

\vspace{-0.35cm}

\caption {Comparison of the relative landmarking strategy and the baseline using the extracted results from the prior evaluations}
\label{tab:compare_landmarking_prior_evaluations}

\centering
%\tiny
\scriptsize


\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{k}  & \textbf{1} & 2 & 3  & \textbf{4}  & 5  & 6  & 7  & \textbf{8}  & 9  & \textbf{10} & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & \textbf{19} & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 \\ \hline
\textbf{c1} & \textbf{0} & 0 & 2  & \textbf{2}  & 3  & 4  & 7  & \textbf{10} & 14 & \textbf{18} & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 & \textbf{20} & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 \\ \hline
\textbf{c2} & \textbf{4} & 8 & 11 & \textbf{12} & 12 & 14 & 14 & \textbf{15} & 16 & \textbf{18} & 18 & 18 & 18 & 18 & 18 & 18 & 18 & 18 & \textbf{20} & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20 \\ \hline
\end{tabular}



\end{table}


==> tables/tab_landmarking_results_similardatasets.tex <==


\begin{table}[htb!]

\vspace{-0.35cm}

\caption {The most similar dataset resulting from the relative landmarking and the evaluation time of the landmarkers}
\label{tab:similar_dataset}

\centering
%\tiny
\scriptsize



\begin{tabular}{|l|l|l|}
\hline
\textbf{Dataset} & \textbf{The most similar dataset} & \textbf{Evaluation time of the landmarkers (minutes)} \\ \hline
abalone          & gisette                           & 0                                                     \\ \hline
adult            & waveform                          & 1                                                     \\ \hline
amazon           & semeion                           & 6                                                     \\ \hline
car              & mnist                             & 0                                                     \\ \hline
cifar10small     & semeion                           & 19                                                    \\ \hline
convex           & mnist                             & 3                                                     \\ \hline
dexter           & amazon                            & 2                                                     \\ \hline
dorothea         & madelon                           & 35                                                    \\ \hline
gcredit          & semeion                           & 0                                                     \\ \hline
gisette          & waveform                          & 20                                                    \\ \hline
kddcup           & secom                             & -                                                     \\ \hline
krvskp           & mnist                             & 0                                                     \\ \hline
madelon          & gisette                           & 1                                                     \\ \hline
mnist            & semeion                           & 14                                                    \\ \hline
secom            & kddcup                            & 0                                                     \\ \hline
semeion          & mnist                             & 0                                                     \\ \hline
shuttle          & mnist                             & 1                                                     \\ \hline
waveform         & semeion                           & 0                                                     \\ \hline
winequality      & mnist                             & 0                                                     \\ \hline
yeast            & semeion                           & 0                                                     \\ \hline
\end{tabular}



\end{table}



==> tables/tab_pipelines_1.tex <==

\begin{landscape}

\begin{table*}[htb!]

\vspace{-0.35cm}

\caption {The best ML pipelines found using different methods to design configuration spaces.}
\label{tab:pipeline_1}

\centering
%\tiny
\scriptsize


\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Dataset}      & \textbf{best known}                                                                                                                                                & \textbf{no avatar}                                                                                                                                                   & \textbf{avatar}                                                                                                                                                     \\ \hline
\textbf{abalone}      & \begin{tabular}[c]{@{}l@{}}CustomReplaceMissingValues  \\ $\rightarrow$ RandomSubset\\ $\rightarrow$ Resample\\ $\rightarrow$ Logistic\\ $\rightarrow$ Bagging\end{tabular}                    & SimpleLogistic                                                                                                                                                       & SMO                                                                                                                                                                 \\ \hline
\textbf{adult}        & J48                                                                                                                                                                & PART                                                                                                                                                                 & PART                                                                                                                                                                \\ \hline
\textbf{amazon}       & \begin{tabular}[c]{@{}l@{}}CustomReplaceMissingValues\\ $\rightarrow$ Normalize\\ $\rightarrow$ RandomSubset\\ $\rightarrow$ NaiveBayesMultinomial\\ $\rightarrow$ RandomSubSpace\end{tabular} & NaiveBayes                                                                                                                                                           & NaiveBayesMultinomial                                                                                                                                               \\ \hline
\textbf{car}          & SMO$\rightarrow$ MultiClassClassifier                                                                                                                                     & SMO                                                                                                                                                                  & SMO                                                                                                                                                                 \\ \hline
\textbf{cifar10small} & \begin{tabular}[c]{@{}l@{}}RandomForest\\ $\rightarrow$ MultiClassClassifier\end{tabular}                                                                                 & DecisionStump                                                                                                                                                        & RandomForest                                                                                                                                                        \\ \hline
\textbf{convex}       & RandomForest $\rightarrow$ AdaBoostM1                                                                                                                                     & VotedPerceptron                                                                                                                                                      & RandomForest                                                                                                                                                        \\ \hline
\textbf{dexter}       & \begin{tabular}[c]{@{}l@{}}DecisionStump\\ $\rightarrow$ AdaBoostM1\end{tabular}                                                                                          & NaiveBayesMultinomial                                                                                                                                                & SGD                                                                                                                                                                 \\ \hline
\textbf{dorothea}     & \begin{tabular}[c]{@{}l@{}}OneR\\ $\rightarrow$ RandomSubSpace\end{tabular}                                                                                               & PART                                                                                                                                                                 & DecisionStump                                                                                                                                                       \\ \hline
\textbf{gcredit}      & LMT $\rightarrow$ Bagging                                                                                                                                                 & SMO                                                                                                                                                                  & SMO                                                                                                                                                                 \\ \hline
\textbf{gisette}      & \begin{tabular}[c]{@{}l@{}}VotedPerceptron\\ $\rightarrow$ RandomSubSpace\end{tabular}                                                                                    & VotedPerceptron                                                                                                                                                      & VotedPerceptron                                                                                                                                                     \\ \hline
\textbf{kddcup}       & -                                                                                                                                                                  & DecisionStump                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}ClassBalancer\\ $\rightarrow$ RemoveOutliers\\ $\rightarrow$ InterquartileRange\\ $\rightarrow$ AttributeSelection\\ $\rightarrow$ Resample $\rightarrow$ PART\end{tabular} \\ \hline
\textbf{krvskp}       & Jrip $\rightarrow$ AdaBoostM1                                                                                                                                             & RandomForest                                                                                                                                                         & J48                                                                                                                                                                 \\ \hline
\textbf{madelon}      & \begin{tabular}[c]{@{}l@{}}PrincipalComponents\\ $\rightarrow$ IBk\\ $\rightarrow$ LogitBoost\end{tabular}                                                                       & Jrip                                                                                                                                                                 & Jrip                                                                                                                                                                \\ \hline
\textbf{mnist}        & \begin{tabular}[c]{@{}l@{}}CustomReplaceMissingValues\\ $\rightarrow$ Center $\rightarrow$ J48 $\rightarrow$ AdaBoostM1\end{tabular}                                                    & -                                                                                                                                                                    & PART                                                                                                                                                                \\ \hline
\textbf{secom}        & \begin{tabular}[c]{@{}l@{}}J48\\ $\rightarrow$ AdaBoostM1\end{tabular}                                                                                                    & \begin{tabular}[c]{@{}l@{}}ClassBalancer\\ $\rightarrow$ EMImputation $\rightarrow$ Normalize\\ $\rightarrow$ PrincipalComponents\\ $\rightarrow$ Kstar $\rightarrow$ MultiClassClassifier\end{tabular} & SimpleLogistic                                                                                                                                                      \\ \hline
\textbf{semeion}      & \begin{tabular}[c]{@{}l@{}}CustomReplaceMissingValues\\ $\rightarrow$ PrincipalComponents $\rightarrow$ SMO\end{tabular}                                                         & SMO                                                                                                                                                                  & SMO                                                                                                                                                                 \\ \hline
\textbf{shuttle}      & RandomForest $\rightarrow$ AdaBoostM1                                                                                                                                     & RandomForest                                                                                                                                                         & RandomForest                                                                                                                                                        \\ \hline
\textbf{waveform}     & \begin{tabular}[c]{@{}l@{}}RemoveOutliers\\ $\rightarrow$ InterquartileRange $\rightarrow$ Normalize\\ $\rightarrow$ SMO $\rightarrow$ AttributeSelectedClassifier\end{tabular}                & LMT                                                                                                                                                                  & SimpleLogistic                                                                                                                                                      \\ \hline
\textbf{winequality}  & RandomForest $\rightarrow$ AdaBoostM1                                                                                                                                     & RandomForest                                                                                                                                                         & Kstar                                                                                                                                                               \\ \hline
\textbf{yeast}        & RandomForest $\rightarrow$ Bagging                                                                                                                                        & RandomForest                                                                                                                                                         & RandomForest                                                                                                                                                        \\ \hline
\end{tabular}




\end{table*}


\end{landscape}

==> tables/tab_pipelines_2.tex <==


\begin{table}[htb!]

\vspace{-0.35cm}


\caption {The best ML pipelines found using different methods to design configuration spaces.}
\label{tab:pipeline_2}

\centering
\tiny
%\scriptsize


\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Dataset}      & \textbf{L-k1}                                                                                                                                                               & \textbf{L-k4}                                                                                                                                                              & \textbf{L-k8}         & \textbf{L-k10}        & \textbf{L-k19}        \\ \hline
\textbf{abalone}      & \begin{tabular}[c]{@{}l@{}}CustomReplaceMissingValues\\ $\rightarrow$ Normalize\\ $\rightarrow$ RandomSubset\\ $\rightarrow$ SimpleLogistic\end{tabular}                                         & \begin{tabular}[c]{@{}l@{}}ClassBalancer\\ $\rightarrow$ RemoveOutliers\\ $\rightarrow$ InterquartileRange\\ $\rightarrow$ Normalize\\ $\rightarrow$ RandomSubset\\ $\rightarrow$ SimpleLogistic\end{tabular} & REPTree               & RandomForest          & PART                  \\ \hline
\textbf{adult}        & \begin{tabular}[c]{@{}l@{}}RemoveOutliers\\ $\rightarrow$ InterquartileRange\\ $\rightarrow$ Center $\rightarrow$ Logistic\end{tabular}                                                          & Logistic                                                                                                                                                                   & NaiveBayes            & PART                  & PART                  \\ \hline
\textbf{amazon}       & \begin{tabular}[c]{@{}l@{}}ClassBalancer\\ $\rightarrow$ RemoveOutliers\\ $\rightarrow$ InterquartileRange\\ $\rightarrow$ Center\\ $\rightarrow$ Logistic\end{tabular}                                 & SMO                                                                                                                                                                        & NaiveBayesMultinomial & NaiveBayesMultinomial & NaiveBayesMultinomial \\ \hline
\textbf{car}          & SMO                                                                                                                                                                         & SMO                                                                                                                                                                        & SMO                   & SMO                   & SMO                   \\ \hline
\textbf{cifar10small} & \begin{tabular}[c]{@{}l@{}}RandomSubset\\ $\rightarrow$ PeriodicSampling $\rightarrow$ Logistic\end{tabular}                                                                              & NaiveBayesMultinomial                                                                                                                                                      & RandomForest          & NaiveBayes            & -                     \\ \hline
\textbf{convex}       & -                                                                                                                                                                           & Jrip                                                                                                                                                                       & SMO                   & RandomForest          & RandomForest          \\ \hline
\textbf{dexter}       & SMO                                                                                                                                                                         & SMO                                                                                                                                                                        & SMO                   & SMO                   & SimpleLogistic        \\ \hline
\textbf{dorothea}     & -                                                                                                                                                                           & -                                                                                                                                                                          & -                     & DecisionStump         & DecisionStump         \\ \hline
\textbf{gcredit}      & LMT                                                                                                                                                                         & NaiveBayes                                                                                                                                                                 & NaiveBayes            & SMO                   & SMO                   \\ \hline
\textbf{gisette}      & Logistic                                                                                                                                                                    & -                                                                                                                                                                          & Jrip                  & RandomForest          & Logistic              \\ \hline
\textbf{kddcup}       & -                                                                                                                                                                           & -                                                                                                                                                                          & -                     & -                     & -                     \\ \hline
\textbf{krvskp}       & SMO                                                                                                                                                                         & SMO                                                                                                                                                                        & J48                   & J48                   & RandomForest          \\ \hline
\textbf{madelon}      & \begin{tabular}[c]{@{}l@{}}SpreadSubsample\\ $\rightarrow$ CustomReplaceMissingValues\\ $\rightarrow$ Normalize $\rightarrow$ RandomSubset\\ $\rightarrow$ Resample $\rightarrow$ VotedPerceptron\end{tabular} & Jrip                                                                                                                                                                       & Jrip                  & Jrip                  & Jrip                  \\ \hline
\textbf{mnist}        & -                                                                                                                                                                           & -                                                                                                                                                                          & -                     & SMO                   & SimpleLogistic        \\ \hline
\textbf{secom}        & -                                                                                                                                                                           & ZeroR                                                                                                                                                                      & ZeroR                 & DecisionTable         & LMT                   \\ \hline
\textbf{semeion}      & SMO                                                                                                                                                                         & SMO                                                                                                                                                                        & SMO                   & SMO                   & SMO                   \\ \hline
\textbf{shuttle}      & SMO                                                                                                                                                                         & Jrip                                                                                                                                                                       & PART                  & RandomForest          & RandomForest          \\ \hline
\textbf{waveform}     & SMO                                                                                                                                                                         & SMO                                                                                                                                                                        & SimpleLogistic        & SimpleLogistic        & LMT                   \\ \hline
\textbf{winequality}  & SMO                                                                                                                                                                         & Kstar                                                                                                                                                                      & SMO                   & RandomForest          & Kstar                 \\ \hline
\textbf{yeast}        & Logistic                                                                                                                                                                    & SMO                                                                                                                                                                        & RandomForest          & RandomForest          & RandomForest          \\ \hline
\end{tabular}


\end{table}


==> tables/tab_pipelines_3.tex <==

\begin{landscape}

\begin{table*}[htb!]

\vspace{-0.35cm}


\caption {The best ML pipelines found using different methods to design configuration spaces.}
\label{tab:pipeline_3}

\centering
%\tiny
\scriptsize


\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Dataset}      & \textbf{O-k1}                                                                                                                                                                                                 & \textbf{O-k4}                                                                                                                               & \textbf{O-k8}         & \textbf{O-k10}        & \textbf{O-k19}        \\ \hline
\textbf{abalone}      & Logistic                                                                                                                                                                                                      & DecisionTable                                                                                                                               & SimpleLogistic        & PART                  & MultilayerPerceptron  \\ \hline
\textbf{adult}        & -                                                                                                                                                                                                             & PART                                                                                                                                        & J48                   & J48                   & PART                  \\ \hline
\textbf{amazon}       & -                                                                                                                                                                                                             & NaiveBayesMultinomial                                                                                                                       & NaiveBayesMultinomial & NaiveBayesMultinomial & NaiveBayesMultinomial \\ \hline
\textbf{car}          & LMT                                                                                                                                                                                                           & SMO                                                                                                                                         & SMO                   & SMO                   & SMO                   \\ \hline
\textbf{cifar10small} & -                                                                                                                                                                                                             & RandomForest                                                                                                                                & RandomForest          & NaiveBayes            & RandomForest          \\ \hline
\textbf{convex}       & -                                                                                                                                                                                                             & RandomForest                                                                                                                                & SMO                   & RandomForest          & RandomForest          \\ \hline
\textbf{dexter}       & SGD                                                                                                                                                                                                           & SGD                                                                                                                                         & VotedPerceptron       & SGD                   & SimpleLogistic        \\ \hline
\textbf{dorothea}     & \begin{tabular}[c]{@{}l@{}}SpreadSubsample\\ $\rightarrow$ CustomReplaceMissingValues\\ $\rightarrow$ Center $\rightarrow$ DecisionStump\end{tabular}                                                                              & NaiveBayes                                                                                                                                  & NaiveBayes            & NaiveBayes            & OneR                  \\ \hline
\textbf{gcredit}      & NaiveBayes                                                                                                                                                                                                    & MultilayerPerceptron                                                                                                                        & SMO                   & MultilayerPerceptron  & MultilayerPerceptron  \\ \hline
\textbf{gisette}      & VotedPerceptron                                                                                                                                                                                               & VotedPerceptron                                                                                                                             & VotedPerceptron       & VotedPerceptron       & VotedPerceptron       \\ \hline
\textbf{kddcup}       & MultilayerPerceptron                                                                                                                                                                                          & Ibk                                                                                                                                         & DecisionStump         & -                     & DecisionStump         \\ \hline
\textbf{krvskp}       & LMT                                                                                                                                                                                                           & J48                                                                                                                                         & J48                   & J48                   & J48                   \\ \hline
\textbf{madelon}      & Jrip                                                                                                                                                                                                          & Jrip                                                                                                                                        & Jrip                  & Jrip                  & Jrip                  \\ \hline
\textbf{mnist}        & SMO                                                                                                                                                                                                           & -                                                                                                                                           & SMO                   & RandomForest          & SMO                   \\ \hline
\textbf{secom}        & \begin{tabular}[c]{@{}l@{}}ClassBalancer\\ $\rightarrow$ CustomReplaceMissingValues\\ $\rightarrow$ RemoveOutliers $\rightarrow$ InterquartileRange\\ $\rightarrow$ Normalize $\rightarrow$ PeriodicSampling\\ $\rightarrow$ DecisionStump\end{tabular} & \begin{tabular}[c]{@{}l@{}}SpreadSubsample\\ $\rightarrow$ Standardize\\ $\rightarrow$ RandomSubset\\ $\rightarrow$ PeriodicSampling\\ $\rightarrow$ ZeroR\end{tabular} & Kstar                 & VotedPerceptron       & Kstar                 \\ \hline
\textbf{semeion}      & Logistic                                                                                                                                                                                                      & SMO                                                                                                                                         & SMO                   & SMO                   & SMO                   \\ \hline
\textbf{shuttle}      & RandomForest                                                                                                                                                                                                  & RandomForest                                                                                                                                & RandomForest          & RandomForest          & RandomForest          \\ \hline
\textbf{waveform}     & Logistic                                                                                                                                                                                                      & SimpleLogistic                                                                                                                              & SimpleLogistic        & SimpleLogistic        & SimpleLogistic        \\ \hline
\textbf{winequality}  & RandomForest                                                                                                                                                                                                  & RandomForest                                                                                                                                & RandomForest          & Kstar                 & Kstar                 \\ \hline
\textbf{yeast}        & RandomForest                                                                                                                                                                                                  & RandomForest                                                                                                                                & RandomForest          & RandomForest          & RandomForest          \\ \hline
\end{tabular}


\end{table*}


\end{landscape}

==> tables/table_investigate_baseline.tex <==


\begin{table}[htb!]

\vspace{-0.35cm}
\captionsetup{font=scriptsize}
\caption {Compare the ranking of the well-performing predictors using the top well-performing predictors of all datasets and top well-performing predictors of the most similar dataset found by the relative landmarking.}
\label{tab:exp_ranking_compare}

\centering
%\tiny
\scriptsize



\begin{tabular}{|l|l|l|}
\hline
\textbf{Dataset}      & \textbf{\begin{tabular}[c]{@{}l@{}}The number of predictors have their rankings \\ in top 8 well-performing predictors of all datasets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}The best ranking in top 8 well-performing\\ predictors of all datasets\end{tabular}} \\ \hline
\textbf{abalone}      & 3                                                                                                                                                    & 5                                                                                                                       \\ \hline
\textbf{adult}        & 5                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{amazon}       & 6                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{car}          & 5                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{cifar10small} & 4                                                                                                                                                    & 3                                                                                                                       \\ \hline
\textbf{convex}       & 4                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{dexter}       & 5                                                                                                                                                    & 4                                                                                                                       \\ \hline
\textbf{dorothea}     & 4                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{gcredit}      & 4                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{gisette}      & 5                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{kddcup}       & 1                                                                                                                                                    & 8                                                                                                                       \\ \hline
\textbf{krvskp}       & 6                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{madelon}      & 6                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{mnist}        & 4                                                                                                                                                    & 4                                                                                                                       \\ \hline
\textbf{secom}        & 1                                                                                                                                                    & 8                                                                                                                       \\ \hline
\textbf{semeion}      & 4                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{shuttle}      & 6                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{waveform}     & 5                                                                                                                                                    & 2                                                                                                                       \\ \hline
\textbf{winequality}  & 5                                                                                                                                                    & 1                                                                                                                       \\ \hline
\textbf{yeast}        & 7                                                                                                                                                    & 1                                                                                                                       \\ \hline
\end{tabular}








\end{table}



